Self-Evolution Learning for Discriminative Language Model Pretraining

Masked language modeling, widely used in discriminative language model (e.g., BERT) pretraining, commonly adopts a random masking strategy. However, random masking does not consider the importance of the different words in the sentence meaning, where some of them are more worthy to be predicted. Therefore, various masking strategies (e.g., entity-level masking) are proposed, but most of them require expensive prior knowledge and generally train from scratch without reusing existing model weights. In this paper, we present Self-Evolution learning (SE), a simple and effective token masking and learning method to fully and wisely exploit the knowledge from data. SE focuses on learning the informative yet under-explored tokens and adaptively regularizes the training by introducing a novel Token-specific Label Smoothing approach. Experiments on 10 tasks show that our SE brings consistent and significant improvements (+1.43~2.12 average scores) upon different PLMs. In-depth analyses demonstrate that SE improves linguistic knowledge learning and generalization.

==> [ACL23] SE4PLMs-Camera_Ready/sections/0_abstract.tex <==
\begin{abstract}
% Masked language modeling (MLM), which is widely used in discriminative language model (e.g., BERT) pretraining, usually suffers from the problem of token imbalance (different tokens appear with different frequencies). The vanilla random masking used in MLM tends to select the high-frequency tokens, but neglect the low-frequency tokens that may carry critical linguistical knowledge, thus leading to sub-optimal performance. In this paper, we propose a simple and effective \textit{Self-Evolution learning} (SE) mechanism to improve over the existing discriminative pretrained language models. The central idea of SE mechanism is to enforce the pretrained models to focus on the learning of low-frequency but informative tokens. To prevent the overfitting on these tokens, we further propose a novel \textit{Token-specific Label Smoothing} regularization approach to promote predictive diversity with self-distillation knowledge. 

Masked language modeling, widely used in discriminative language model (\textit{e.g.}, BERT) pretraining, commonly adopts a random masking strategy. However, random masking does not consider the importance of the different words in the sentence meaning, where some of them are more worthy to be predicted. Therefore, various masking strategies (\textit{e.g.}, entity-level masking) are proposed, but most of them require expensive prior knowledge and generally train from scratch without reusing existing model weights. In this paper, we present \textit{Self-Evolution learning} ($\mathbb{SE}$), a simple and effective token masking and learning method to fully and wisely exploit the knowledge from data. $\mathbb{SE}$ focuses on learning the informative yet under-explored tokens and adaptively regularizes the training by introducing a novel \textit{Token-specific Label Smoothing} approach. Experiments on 10 tasks show that our $\mathbb{SE}$ brings consistent and significant improvements (+1.43$\sim$2.12 average scores) upon different PLMs. In-depth analyses demonstrate that $\mathbb{SE}$ improves linguistic knowledge learning and generalization.
%chatGPT version:↓
% In recent years, masked language modeling (MLM), commonly used in discriminative language model pretraining such as BERT, has become popular. However, the standard approach of randomly masking words in a sentence does not take into account the importance of different words in determining the meaning of the sentence. To mitigate this limitation, various masking strategies, such as entity-level masking, have been proposed, but most of them are computationally expensive and require training from scratch. In this paper, we propose Self-Evolution learning (SE), an efficient and effective token masking and learning method that fully leverages the knowledge in the data. SE focuses on learning the informative yet under-explored tokens and reduces overfitting by introducing a novel Token-specific Label Smoothing approach. Through experiments on 10 tasks, we show that SE consistently improves the performance of various state-of-the-art models by an average of 1.01-1.61 points. In-depth analyses also demonstrate that SE improves linguistic knowledge learning and generalization.
% random masking may neglect the impact of different tokens, 
% for example, the tokens ``\textit{Bush}'', ``\textit{talk}'', and ``\textit{Sharon}'' contain more linguistic information than ``\textit{a}'' in a sample sentence ``\textit{Bush held a talk with Sharon}''. 
% Hence, several carefully-designed masking strategies (e.g., entity-level masking) are recently proposed, but most of them require external resources or supervision and are generally used to train the models from scratch without reusing the existing pretrained models.
% In this paper, we propose a simple and effective \textit{Self-Evolution learning} (SE) mechanism, which can fully explore the abilities of the existing pretrained models without using any external resource or supervision.
% by enforcing the models to learn the informative (but under-explored) patterns.
% The key idea of $\mathbb{SE}$ is to enforce the models to dynamically focus on the learning of informative but under-explored tokens. 
% To prevent overfitting to these tokens, we introduce a novel \textit{Token-specific Label Smoothing} approach to adaptively regularize the training for each masked token.
% Furthermore, to prevent the overfitting to these tokens, we propose a novel \textit{Token-specific Label Smoothing} approach to adaptively regularize the training for each masked token.
% promoting predictive diversity with self-distillation knowledge. 
% Specifically, SE mechanism is a two stage process: \textit{self-questioning} and \textit{self-evolution training}, where the first is to select the informative tokens wisely predicted by the pretrained model itself, and the second is to supervise the MLM process with calibrated token-specific smooth labels.
\end{abstract}

==> [ACL23] SE4PLMs-Camera_Ready/sections/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
Masked language modeling (MLM), which commonly adopts a random masking strategy to select the mask tokens, has become the \textit{de-facto} standard for discriminative pretrained language models (PLMs)~\cite{devlin2019bert,liu2019roberta,he2020deberta,joshi2020spanbert}. However, such a random masking process is usually criticized as being sub-optimal, as it allocates an equal masking rate for all tokens. In particular, the masked tokens are sometimes too easy to guess with only local cues or shallow patterns~\cite{joshi2020spanbert}, while the informative tokens that carry more critical linguistic knowledge may be neglected~\cite{church1990word,sadeq2022informask}.
For example, ``\textit{Bush}'' and ``\textit{Sharon}'' express more important meaning than ``\textit{a}'' in the sample sentence ``\textit{Bush held a talk with Sharon}''. MLM with predicting the above easy-to-guess tokens, \textit{e.g.}, ``a'', would lead to low data efficiency and sub-optimal model capability. %capacity.

To address this problem, various methods have been carefully designed to improve MLM via fully leveraging the training data~\cite{sun2019ernie,joshi2020spanbert,levine2020pmi}.
% Hence, several carefully-designed masking strategies are recently proposed to improve the MLM~\cite{sun2019ernie,joshi2020spanbert,levine2020pmi} 
% such as entity-level masking~\cite{sun2019ernie}, span-level masking~\cite{joshi2020spanbert} and N-grams masking~\cite{levine2020pmi}
The common goal is to inject language prior knowledge into the pretraining process~\cite{cui2022lert,ding2021understanding}. Although empirically successful, there are still some limitations. 
First, they usually require annotation derived from off-the-shelf tools to select mask tokens, which is not only expensive but also too deterministic\footnote{The once-for-all prior is not suitable for different PLMs, \textit{e.g.}, under-explored word for BERT may already well-mastered by RoBERTa.}, and may cause error propagation from the third-party tool.
For instance, \citet{sun2019ernie} employ external linguistic tools, \textit{e.g.}, Stanford CoreNLP~\cite{manning2014stanford}, to annotate the entities.
Second, to ensure the effectiveness of the masking strategy, most previous works train PLM from scratch without reusing the existing models trained with vanilla MLM~\cite{sun2019ernie,joshi2020spanbert,levine2020pmi,sadeq2022informask}, which is wasteful and inefficient.
% First, these strategies usually require external resources or supervision to select the tokens that should be masked. For example, for entity-level masking~\cite{sun2019ernie}, it is usually necessary to use external linguistic tools (e.g., Stanford CoreNLP~\cite{manning2014stanford}) to recognize the named entities. 
% On the other hand, to ensure the effectiveness of the proposed masking strategy, most previous works train the models from scratch without reusing the existing models trained with the vanilla MLM, which is wasteful and inefficient. 

Thus, there \textbf{raises a question}:
% \begin{tcolorbox}
%     \begin{center} 
%     {\sf whether we can strengthen the existing PLM capacity and data efficiency through learning from the informative yet under-explored tokens, where such tokens are determined by the PLM itself rather than the expensive third-party tool.}
%     \end{center} 
% \end{tcolorbox}
\textit{whether we can strengthen the PLM capability and data efficiency through further learning from the informative yet under-explored tokens, where such tokens are determined by the existing PLM itself.
}
In fact, an off-the-shelf PLM already has the ability to determine the worthy and informative tokens that should be further exploited, as the representation of PLM generally can reveal good enough linguistic properties~\cite{hewitt-manning-2019-structural,swayamdipta-etal-2020-dataset}. For example, tokens that PLMs predict incorrect or low confidence are usually more hard-to-learn and challenging, which are essential for further training. Also, the conjecture to improve the off-the-shelf PLM is model-agnostic, green, and efficient, thus having the great potential to evolve any existing discriminative PLMs.

% Thus, this raises the question that \textit{whether we can fully explore the abilities of the existing PLMs by enforcing them to further learn the linguistic knowledge from the pretraining data in a self-motivated manner}.
% In fact, an off-the-shelf PLM already has the ability to determine which tokens are informative and worthy to be further learned, as its behavior on tokens can reveal the linguistic characteristics~\cite{swayamdipta-etal-2020-dataset}. For example, the tokens that PLMs predict with low correctness or confidence are usually more hard-to-learn and challenging
% \footnote{We refer to these challenging tokens that are not learned well by PLMs as the informative but under-explored tokens.}
% , which are essential for the further training of PLMs.
% the existing PLMs already have the ability to determine which tokens are worthy to be masked, as the tokens that PLMs predict with low correctness or confidence are usually more hard-to-learn and challenging\footnote{We refer to these challenging tokens that are not learned well by PLMs as the informative but under-explored tokens.}, which are essential for further training of PLMs~\cite{swayamdipta-etal-2020-dataset}. Thus, this raises the question that \textit{whether we can fully explore the abilities of the existing PLMs by encouraging them to wisely select the informative but under-explored tokens and learn from these tokens.}
% encouraging them to further learn the useful (but under-explored) knowledge from the pretraining data without using any external resources or supervision}.
% \textit{whether we can encourage the existing pretrained models to wisely select the informative but under-explored tokens and learn from these tokens.}

Motivated by this, we design a simple and effective \textit{Self-Evolution learning} ($\mathbb{SE}$) mechanism to improve the pretraining of discriminative PLMs. Specifically, the $\mathbb{SE}$ contains two stages: \ding{182}\textit{self-questioning} and \ding{183}\textit{self-evolution training}. In \textbf{stage~1}, the PLM is forced to locate the informative but under-explored tokens\footnote{We refer to those hard-to-learn tokens that are not learned well by PLMs as the informative but under-explored tokens.} from the pretraining data.
% , which the PLM tends to predict wrongly (i.e., different from the ground-truths) or indeterminately.
% More specifically, given a sentence as input, the MLM head of PLM will output the probability distributions of the vocabulary size for each token position. As expected, most of probability distributions are as close as possible to the ground-truth one-hot representations. However, for some low-frequency but informative tokens, since they are less likely to be learned during pretraining, the PLM may predict with less confidence or correctness. These under-explored tokens usually carry more critical linguistic knowledge and are worthy to be further learned.
%没啥信息量可以去掉
% In practice, to estimate the information and complexity of tokens, we introduce two simple metrics that are model-dependent (i.e., these metrics are based on the behavior of PLMs on individual tokens in the sentences, which can reveal tokens with distinct pronounced characteristics) and do not require any external resources.
%没啥信息量可以去掉
% In this way, we can select these informative tokens for masking and then encourage the PLM to learn from these informative tokens, thus continuously improving the capability of the PLM. 
After locating these hard-to-learn tokens, we then encourage the PLM to learn from them in \textbf{stage~2}, where we basically follow the vanilla MLM to mask these tokens and then optimize the PLM by minimizing the loss between the predictions and one-hot labels.
It should be noted that due to the hard-to-learn properties, directly enforcing the PLM to fit the hard labels may lead to overfitting or overconfidence problem~\cite{miao-etal-2021-prevent}.
% Intuitively, we can follow the vanilla MLM process, i.e., masking these tokens first and then training the PLM by minimizing the loss between the predictions and one-hot labels for the masked tokens. 
% However, as these tokens are more hard-to-learn and challenging, enforcing the PLM to remember the hard target labels will lead to overfitting or overconfident problems~\cite{li2022pre}. 
% On the other hand, considering the diversity of these tokens, if we force the PLM to promote one specified ground truth over others, the other reasonable ``ground truths'' (for a given masked token, there can be more than one reasonable prediction) become false negatives that may plague the training process or cause a performance decrease~\cite{li2022pre}.
Inspired by the label smoothing (LS)~\cite{szegedy2016rethinking} that regularizes the learning by smoothing target labels with a pre-defined (static) prior distribution, we propose a novel \textit{Token-specific Label Smoothing} (TLS) approach. Our TLS considers both the precise hard label and, importantly, the \textit{easily-digestible}\footnote{Analogous to human learning behavior, it is often easier for humans to grasp new things described by their familiar knowledge~\cite{reder2016building}.} distribution that is adaptively generated by the PLM itself.

%这段揭示方法合理性，适合放到方法说
% Specifically, as~\citet{yuan2020revisiting} proved, the smoothed label in LS can be split into two parts, where the first is used to perform the ordinary cross-entropy between predictions and one-hot labels, and the second corresponds to a virtual teacher which provides a prior distribution to teach the model. In the vanilla LS, the uniform distribution is usually used as the prior distribution, which we argue is sub-optimal, as the uniform one can hardly provide linguistic information for training. 
% Hence, in our TLS, we view the second part in LS as a knowledge distillation (KD) process and adopt a more informative distribution, which contains more linguistic ``dark'' knowledge, as a virtual teacher to adaptively guide the training of PLM on the masked tokens. 
% More specifically, we get inspiration from the self-distillation~\cite{zhang2019your} and use the distribution of tokens (on corresponding masked positions) in the original sentence (without corrupting) predicted by the model itself as the teacher distribution.
% predictions on the original sentence (without corrupting) from the model as a virtual teacher model to guide the training of student (i.e., the model itself) on the masked tokens. In general, motivated by the relationships between KD and LS, we recast the uninformative uniform distribution used in vanilla LS with an adaptive KD-based distribution that contains more linguistic ``dark'' knowledge.

% Instead of using static smoothing label distribution, our TLS adaptively controls the smoothing extent for each masked token by adopting the token-specific distributions that contain more linguistic knowledge. 
% \textcolor{red}{Does not explain the details? Reviewers may be confused by TLS approach, especially why it contains linguistic knowledge?}. 
% With such an adaptive regularization approach, the $\mathbb{SE}$ mechanism can alleviate the difficulty of learning from these hard-to-learn and informative tokens, and improve the generalization of PLMs effectively.
% Specifically, considering that the original probabilities of these informative token predicted by PLM before masking may contain some linguistic knowledge as well, we can refer to these informative probabilities as the ``teacher predictions'' and then use them as the prior label distributions to calibrate the smoothing label. With the regularization effect of token-specific smoothing label, the PLMs can effectively learn the linguistical knowledge from the informative tokens.

% We conduct a large-scale and systematic study to evaluate the effectiveness of the $\mathbb{SE}$ mechanism. 
We validated our $\mathbb{SE}$ on several benchmarks including GLUE~\cite{wang2018glue}, SuperGLUE~\cite{wang2019superglue}, SQuAD2.0~\cite{rajpurkar2018know}, SWAG~\cite{zellers-etal-2018-swag} and LAMA~\cite{petroni2019language} over several PLMs: BRET~\cite{devlin2019bert}-\textsc{Base}, -\textsc{Large}, RoBERTa~\cite{liu2019roberta}-\textsc{Base}, and -\textsc{Large}. Experiments demonstrate the effectiveness and universality of our approach.
Extensive analyses confirm that $\mathbb{SE}$ effectively enhances the ability of PLMs on linguistic knowledge learning, model generalization and robustness.
\paragraph{Contributions}Our main contributions are:
\begin{itemize}
    \item We propose $\mathbb{SE}$ to strengthen the MLM-based PLMs, where our mechanism does not require external tools and enjoys a simple recipe: continue pretraining with $\mathbb{SE}$.
    \item We design a novel token-specific label smoothing approach for regularization, which adopts the token-specific knowledge-intensive distributions to adaptively smooth the target labels.
    \item Extensive experiments show that our $\mathbb{SE}$ could significantly and robustly evolve a series of backbone PLMs, up to +2.36 average score improvement on GLUE benchmark upon RoBERTa.
\end{itemize}

% We apply the $\mathbb{SE}$ upon 4 representative discriminative PLMs and evaluate on 10 tasks, including GLUE~\cite{wang2018glue}, SuperGLUE~\cite{wang2019superglue}, SQuAD2.0~\cite{rajpurkar2018know}, and SWAG~\cite{zellers-etal-2018-swag} benchmarks, where the results show that $\mathbb{SE}$ significantly and consistently improves the PLMs by 1.01$\sim$1.61 average score. Additionally, quantitative analysis and in-depth discussion demonstrate that $\mathbb{SE}$ can enhance the ability of PLMs on linguistic knowledge learning, and improve the model generalization and robustness effectively. 
% To summarize, \textbf{our contributions} are as follows: (1) we propose a novel self-evolution mechanism to fully explore the abilities of existing discriminative PLMs, where the $\mathbb{SE}$ mechanism does not require any external resources or supervision and improves the efficiency of pretraining by reusing the existing PLMs. (2) We propose a novel token-specific label smoothing approach for MLM training regularization, which adopts the token-specific knowledge-intense distributions to adaptively smooth the target labels. (3) Extensive experiments show that $\mathbb{SE}$ brings consistent and significant improvements among several PLMs. The systematic study demonstrates that $\mathbb{SE}$ could enhance the ability of knowledge learning and model generalization.

==> [ACL23] SE4PLMs-Camera_Ready/sections/2_related_work.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.95\textwidth]{method.pdf}
    \caption{\label{fig:self-evolution}Overview of the proposed $\mathbb{SE}$ mechanism, which contains two stages: \ding{182} using an existing PLM to locate the informative yet under-explored tokens and \ding{183} encouraging the PLM to robustly learn from these tokens via a token-specific label smoothing approach. 
    % The \textbf{stage 1} is to enforce an off-the-shelf PLM to locate the informative yet under-explored tokens from the pretraining data, while the second aims to encourage the PLM to robustly learn from these tokens via a novel token-specific label smoothing regularization approach.
    }
\end{figure*}

\section{Related Works}
\label{sec:related}
In recent years, we have witnessed numerous discriminative PLMs~\cite{devlin2019bert,liu2019roberta,he2020deberta,sun2019ernie,joshi2020spanbert} that achieved tremendous success in various natural language understanding (NLU) tasks. Although the discriminative PLMs vary in terms of pretraining data or model architecture, they are commonly based on MLM loss function. MLM mechanism is pioneered in BERT~\cite{devlin2019bert} that uses a random masking strategy to mask some tokens, and then enforces the PLM to learn to recover word information from the masked tokens. Obviously, the vanilla MLM is a linguistic-agnostic task, as the random masking procedure does not integrate linguistic knowledge explicitly, which is sub-optimal. Thus, several previous studies attempt to improve MLM by exploring a diverse of linguistically-motivated masking strategies, such as entity-level masking~\cite{sun2019ernie}, span-level masking~\cite{joshi2020spanbert}, N-grams masking~\cite{levine2020pmi}, \textit{etc.}, to fully leverage the pretraining data. 
% In practice, MLM select a subset of tokens from a sentence and then replace them with a special mask token, i.e., \texttt{[MASK]}. Lastly, a PLM is forced to predict the ground-truths for the masked tokens based on the context. 

Although achieving remarkable performance, these strategies still have some limitations. First, their implementations are relatively complex, as they usually require annotation derived from external models or tools to select tokens for masking.
Even for the unsupervised PMI-masking~\cite{sadeq2022informask}, it is still expensive to measure the pointwise mutual information for pretrain-level large-scale data, and the annotated labels are static, while our $\mathbb{SE}$ could obtain dynamic annotations via given existing PLMs.
% Although the recently proposed PMI-masking method~\cite{sadeq2022informask} is fully unsupervised, the process to measure the pointwise mutual information is still relatively complex. 
Second, in order to ensure the effectiveness of masking strategy, most previous works~\cite{sun2019ernie,joshi2020spanbert,levine2020pmi,sadeq2022informask} train the language models from scratch without reusing the existing PLMs trained with vanilla MLM, which is wasteful and inefficient.

Along the same research line, in this paper, we improve the MLM-based PLMs with a novel self-evolution learning mechanism. Instead of training a PLM from scratch based on a carefully-designed and complex masking strategy, our mechanism aims to strengthen the PLM's capability and data efficiency by further learning from the informative yet under-explored tokens, which are determined by the existing PLM itself.
% We fully explore the abilities of existing discriminative PLMs by encouraging them to learn from the informative but under-explored tokens. By enforcing the PLMs to continuously learn the patterns that are under-explored, we can improve the performance on downstream tasks effectively.


==> [ACL23] SE4PLMs-Camera_Ready/sections/3_methods.tex <==

\section{Methodology}
% In this section, we first review the MLM and then introduce the proposed $\mathbb{SE}$ mechanism.
\label{sec:method}
\subsection{Preliminary}
Given a sentence $S=\{t_1,t_2,...,t_n\}$ with $n$ tokens, MLM first randomly selects some percentage of the input tokens and replaces them with a special mask symbol \texttt{[MASK]}. Suppose that there are $m$ masked tokens and $\{k_1,k_2,...,k_m\}$ is the set of masked positions, we can denote the masked tokens as $M=\{t_{k_1},t_{k_2},...,t_{k_m}\}$. Let $S'$ denote the masked sentence, we can feed $S'$ into the model and obtain the last hidden layer representations as $H \in \mathbb{R}^{n \times d}$ ($d$ is the hidden size), and a subset of representations w.r.t masked positions as $H^m \in \mathbb{R}^{m \times d}$. Subsequently, the input word embedding matrix $E \in \mathbb{R}^{V \times d}$ ($V$ is the vocabulary size) is used to project the hidden representations into vocabulary space. Lastly, we can get the normalized prediction probabilities for each masked token as:
\begin{align}
    p_i=\text{softmax}(H^m_i E^T+ b),
\end{align}
where $p_i \in \mathbb{R}^V$ and $ i\in\{1,2,...,m\}$.
Finally, given the one-hot labels $y_i$, we use the cross-entropy loss to optimize the MLM task:
\begin{align}
    \mathcal{L}_{MLM}=-\frac{1}{m}\sum_{i=1}^m y_i \log p_i
    \label{mlm_loss}
\end{align}

\subsection{Self-Evolution Learning for PLMs}
\label{sec:se_method}
In this part, we introduce our $\mathbb{SE}$ mechanism in detail. At its core, $\mathbb{SE}$ is to enforce the existing PLM to further learn from the informative yet under-explored tokens, which are wisely determined by the PLM itself.
Figure~\ref{fig:self-evolution} illustrates the process of $\mathbb{SE}$ mechanism, which contains two stages: (1) \textit{self-questioning} and (2) \textit{self-evolution training}. 
% At its core, $\mathbb{SE}$ is to strengthen an existing PLM's capacity through enforcing it to further learn from the informative yet under-explored tokens, which are determined by the PLM itself.
% Instead of training the models from scratch, self-evolution learning aims to encourage the existing ``naive'' PLMs\footnote{We denote the PLMs trained with the vanilla MLM task as the ``naive'' PLMs.} to find patterns (tokens) that are not learned well but are more informative, and then fix them. The illustration of self-evolution learning can be seen in Figure~\ref{fig:self-evolution}. Specifically, there are two stages in our self-evolution learning, as follows.

\paragraph{\ding{182} Self-questioning Stage.}
The goal of this stage is to select the informative yet under-explored tokens, \textit{i.e.}, these hard-to-learn tokens that the PLMs do not learn well during the previous pretraining. However,
\textit{how to select these target tokens?} Inspired by the finding of the representations of the off-the-shelf PLM on individual tokens can reveal good enough linguistic properties~\cite{hewitt-manning-2019-structural,swayamdipta-etal-2020-dataset}, we hereby propose to straightforwardly leverage the behavior of PLMs to wisely select target tokens in this stage.
% Most previous works~\cite{sun2019ernie,cui2021pre} tend to adopt third-party models/tools to do that, which we argue is relatively complex and inefficient. 
% In fact, as shown in the prior studies~\cite{}, the representations of an off-the-shelf PLM on individual tokens can reveal good enough linguistic properties, which can be used to determine these informative yet under-explored tokens
% an off-the-shelf PLM already has the ability to determine these informative yet under-explored tokens, as its representations on individual tokens can reveal good enough linguistic properties.
Specifically, we mainly focus on two important properties, \textit{i.e.}, \textbf{\textit{correctness}} (accuracy) and \textbf{\textit{confidence}} (the probability output that the model assigns to the prediction), as the tokens that PLMs predict incorrect or low confidence are usually more hard-to-learn and worthy for further exploring~\cite{guo2017calibration,park2022calibration}.
Based on the above two properties, we introduce two simple metrics to estimate the learning value of tokens:
% the prior works~\cite{guo2017calibration,park2022calibration} have proved that the \textbf{\textit{confidence}} (the probability output that a model assigns to a prediction) and \textbf{\textit{correctness}} (accuracy) of a sample predicted by a model can reveal samples with distinct pronounced characteristics (i.e., whether they are easy-to-learn or hard-to-learn for the model). Motivated by this, we propose to leverage the behavior (correctness or confidence) of a PLM on individual tokens to wisely predict the informative tokens and introduce several simple metrics to perform the process as below. 

\textbf{Correctness-based metric.} In practice, we first feed the original sentence $S$ into the existing frozen PLM and enforce it to output the prediction probabilities $p_i$ ($i\in\{1,2,...,n\}$) for each token. Given the one-hot labels $y_i$ ($i\in\{1,2,...,n\}$), we calculate the cross-entropy loss (\textit{i.e.}, correctness) for each token position (denoted as $\{l_1,l_2,...,l_n\}$). Then, we set a loss threshold $\mathcal{T}_l$ and select the tokens that exceed $\mathcal{T}_l$ as the target tokens, \textit{i.e.}, $M=\{t_i|l_i>\mathcal{T}_l\}$ where $i\in\{1,2,...,n\}$.

\textbf{Confidence-based metric.} Similarly, we can measure the confidence of tokens and use it as the metric. Different from the above process, in this metric, we compute the entropy of $p_i$ as the confidence for each token (denoted as $\{e_1,e_2,...,e_n\}$). Intuitively, the tokens with high entropy value are hard-to-learn, as the PLM predict them with low confidence towards the gold labels. Also, an entropy threshold $\mathcal{T}_e$ is used to select the target tokens, \textit{i.e.}, $M=\{t_i|e_i>\mathcal{T}_e\}$\footnote{
In practice, 
% we use the Correctness-based metric as the default setting. 
$\mathcal{T}_l$ and $\mathcal{T}_e$ are empirically set as 0.1 and 1, respectively. The detailed analyses are shown in Appendix~\ref{appendix_parameter_analysis}. 
% respectively.
}. 


% In practice, we first feed the original sentence $S$ into a frozen PLM and enforce it to output the prediction probabilities $p_i$ for each token, i.e., $i\in\{1,2,...,n\}$. As the PLM has seen these samples and learned from them in the pretraining stage, it can make deterministic and correct predictions for most of the tokens. 
% That is, let $t^*_i$ denote the predicted token, we have $t^*_i=t_i$ for most of token positions. 
% However, for some tokens, such as ``\texttt{American}'' in the sentence ``\texttt{Thomas Edison was an American inventor and businessman}'', the PLM tends to predict this token as ``\texttt{excellent}'' (the probability of ``excellent'' is 0.44, while the probability of ``American'' is 0.4). We attribute this phenomenon to the fact that the ``\texttt{excellent}'' appears more frequently than the ``\texttt{American}'' during pretraining, which cause the PLM to have a preference for ``\texttt{excellent}'' token. We refer to these informative but under-explored tokens as neglected tokens. 

% To quantitatively select the neglected tokens, we adopt a token-specific metric to measure the uncertainty for each token. The metric could be based on the cross-entropy loss, i.e., we compute the cross-entropy loss for each token and select the tokens that exceed the set loss threshold $\mathcal{T}$ as neglected tokens. Also, we can also compute the entropy for each token and use the entropy-based metric to select neglected tokens.\footnote{The analysis of different metric can be found in section~\ref{sec_abalation_metric}. Note that we use the loss-based metric as the default setting and empirically set the loss threshold $\mathcal{T}$ as 0.1.} After all training samples are fed into the PLM, we can obtain a set of neglected tokens for each training sample. Note that this procedure is conducted offline and does not update the parameters of the original PLM.
% does not learn this knowledge-intense pattern but only makes its prediction based on the local cues.


\paragraph{\ding{183} Self-evolution Training Stage.} After estimating these hard-to-learn tokens, we can then choose them for masking and encourage the PLM to learn from them. Intuitively, we can follow the vanilla MLM process to optimize the PLM by minimizing the loss between the predictions and one-hot labels, as implemented in Eq.~\ref{mlm_loss}. However, due to the hard-to-learn properties of these tokens, directly enforcing the PLM to fit the hard labels may lead to overfitting or overconfidence problem~\cite{miao-etal-2021-prevent,li2022pre}. To tackle this issue, in this stage, inspired by the label smoothing (LS) regularization approach~\cite{szegedy2016rethinking}, we further propose a novel \textit{token-specific label smoothing} (TLS) approach to adaptively regularize the training and improve the generalization of PLMs.

Mathematically, in LS approach, it minimizes the cross-entropy between modified label distribution $y'_i$ and the model output $p_i$, where $y'_i$ is the smoothed label distribution formulated as:
\begin{align}
y'_i=(1-\lambda)*y_i+\lambda*u_i,
\label{eq_ls}
\end{align}
where $u_i$ is a fixed distribution that is usually a uniform distribution, and $\lambda$ is a weighting factor. Furthermore, following~\citet{yuan2020revisiting}, we reformulate the loss function of LS as:
\begin{align}
\mathcal{L}_{LS}=(1-\lambda)*H(y, p)+\lambda*D_{kl}(u,p),
\end{align}
where $H$ denotes the ordinary cross-entropy loss and $D_{kl}$ denotes the KL divergence loss. We can regard $D_{kl}(u,p)$ as a knowledge distillation process, where $u$ corresponds to a virtual teacher to guide the student model (\textit{i.e.}, the PLM). Obviously, it is sub-optimal as $u$ hardly provides enough linguistic information to guide the training of PLM. 

Motivated by this, in our TLS, we design a more informative prior distribution to smooth the labels. 
Specifically, inspired by human learning behavior (it is often easier for humans to grasp new things described by their familiar knowledge~\cite{reder2016building}), we improve the $D_{kl}$ supervision with a more easily-digestible and informative distribution that is adaptively generated by the PLM itself. In other words, $D_{kl}$ can be recast as a self-distillation process, where the virtual teacher distribution is acquired from the student model itself. In practice, for each masked position $k_i$, in addition to the prediction probabilities $p_i$ on the corrupted $S'$, we also feed the original sentence $S$ into the current PLM and regard the corresponding probabilities as the reference probabilities $r_i$\footnote{It is noteworthy that, although the $r_i$ may not be much close to the ground-truths, the linguistic information contained in $r_i$ is potentially beneficial for further learning.}. 
% (referred to as reference probabilities $r_i$). 
% Specifically, motivated by the success of self-distillation~\cite{zhang2019your,zhang2020self}, we regard the prediction on the original sentence $S$ of PLM as the teacher prediction and use it to guide the training of PLM itself on the corrupted sentence $S'$. In practice, for each masked position $k_i$, in addition to the prediction probabilities $p_i$ on the corrupted $S'$, we obtain the reference probabilities $r_i$ via feeding $S$ into the PLM. 
Then, similar to Eq.~\ref{eq_ls}, we can obtain the smoothed label $\Tilde{y}_i$ via:
\begin{align}
\Tilde{y}_i=(1-\lambda)*y_i+\lambda*r_i
\label{label_smoothing}
\end{align}
Lastly, we use the cross-entropy as the loss function in the $\mathbb{SE}$ training stage, as follows:
\begin{align}
    \mathcal{L}_{SE}=-\frac{1}{m}\sum_{i=1}^m \Tilde{y}_i \log p_i
    \label{se_loss}
\end{align}

% \citet{szegedy2016rethinking} first propose the label smoothing approach to regularize the predictive uncertainty of models by smoothing the one-hot label $y$ with a pre-defined label distribution. The prior label distribution is usually a uniform distribution and remains unchanged throughout training in all samples. 

% Intuitively, we can make the PLM learn how to predict these tokens, by minimizing the loss between the predicted probabilities and one-hot labels, as achieved in Eq.~\ref{mlm_loss}. However, considering the learning difficulty of these neglected tokens, directly enforcing the PLM to remember them may lead to the overfitting problem. On the other hand, since there may be more than one reasonable prediction for a masking token, enforcing the PLM to promote one specified ground truth over others will make the other reasonable predictions become false negatives that may plague the training process or cause a performance decrease~\cite{li2022pre}. 

% To tackle this issue, we propose a novel \textit{token-specific label smoothing} approach to adaptively regularize the training and improve the generalization of PLMs. \citet{szegedy2016rethinking} first propose the label smoothing approach to regularize the predictive uncertainty of models by smoothing the one-hot ground-truth label $y$ with a pre-defined prior label distribution. The prior label distribution is usually a uniform distribution and remains unchanged throughout training in all samples. Such a vanilla label smoothing is sub-optimal, as the prior studies~\cite{zhang2020self,yuan2020revisiting} prove that the label smoothing can be viewed as a minimization of KL divergence between the model prediction and the pre-defined prior label distribution, but the uniform distribution may hardly provide enough information for better training. 

% Based on the above motivations, we propose to recast the label smoothing approach with a token-specific informative prior label distribution. Specifically, for each masked position $k_i$, in addition to the prediction probabilities $p_i$, we can also obtain the reference probabilities $r_i$ by feeding the original sentence $S$ into the PLM. We state that the reference probabilities $r_i$ contain some linguistic information and can be used to calibrate the model prediction $p_i$. In other views, we can refer to $r_i$ as a teacher prediction in a self-distillation manner. Intuitively, we can use the $r_i$ as the prior label distribution in the label smoothing approach. Different from the vanilla label smoothing that employs a token-agnostic prior label distribution, our token-specific label smoothing approach can adaptively regularize the training for each masked token and achieve better performance by utilizing the self-distillation knowledge.
% In practice, we merge the $r_i$ and the one-hot label $y_i$ as:
% \begin{align}
% \Tilde{y}_i=(1-\lambda)*y_i+\lambda*r_i
% \label{label_smoothing}
% \end{align}
% where $\Tilde{y}_i$ denotes the smoothing label probabilities and $\lambda$ is a weighting factor that is empirically set as 0.1. Finally, we use the cross-entropy loss function to minimize the difference between $p_i$ and $\Tilde{y}_i$. In this way, different from the strong-headed supervision of the one-hot labels $y_i$, the PLM can benefit more from the smooth and informative labels $\Tilde{y}_i$. 

==> [ACL23] SE4PLMs-Camera_Ready/sections/4_experiments.tex <==
\input{tables/main_results.tex}

\section{Experiments}
\label{sec:experiments}
\subsection{Tasks and Datasets}
% Empirically, following many previous works~\cite{bahri-etal-2022-sharpness,zhong2022e2s2,zhong2022improving},
% To investigate the effectiveness and universality of $\mathbb{SE}$, 
We follow many previous studies~\cite{zhong2022panda,zhong2022toward,zhong2023revisiting,zhong2023bag} and conduct extensive experiments on various NLU tasks, including a diversity of tasks from GLUE~\cite{wang2018glue} and SuperGLUE~\cite{wang2019superglue} benchmarks, \textit{i.e.}, linguistic acceptability (CoLA), natural language inference (RTE, CB), paraphrase (MRPC), question answering (BoolQ), word sense disambiguation (WiC) and causal reasoning (COPA). Additionally, we also evaluate on three knowledge-intense tasks, which require the ability of commonsense knowledge reasoning, \textit{i.e.}, SQuAD2.0~\cite{rajpurkar2018know}, SWAG~\cite{zellers-etal-2018-swag} and LAMA~\cite{petroni2019language}.
In practice, we report the performance with Accuracy (``\textit{Acc.}'') metric for most tasks, except the Matthew correlation (``\textit{Mcc.}'') for CoLA, the F1 and Exact Match (``\textit{EM}'') scores for SQuAD2.0, and the Mean Reciprocal Rank (``\textit{MRR}'') scores for LAMA.
We report the averaged results over 10 random seeds to avoid stochasticity.
The details of all tasks and datasets are provided in Appendix~\ref{appendix_data}.


\subsection{Implementation Details}
\paragraph{Pre-training.} We employ the representative BRET~\cite{devlin2019bert}-\textsc{Base}, -\textsc{Large}, RoBERTa~\cite{liu2019roberta}-\textsc{Base}, and -\textsc{Large} as the backbone discriminative PLMs, and implement our methods in a continued pretraining manner. For pretraining settings, we follow the original papers~\cite{devlin2019bert,liu2019roberta} and use the same pretraining corpus and (most of) hyper-parameters\footnote{Notably, for the continued pretraining process, we use 1/10 of the learning rate in the original paper as the initial one.} (e.g., batch size and the maximum length of the input sentence), respectively.

Especially, as suggested by~\citet{liu2019roberta}, we do not use the next sentence prediction (NSP) objective during BERT pretraining. For our methods, we continue pretraining the backbone PLMs with 2 epochs. Additionally, for reference, we train the PLMs with the vanilla MLM for the same steps and refer to them as the baselines.

\paragraph{Fine-tuning.} The learning rate is selected in \{1e-5, 2e-5, 3e-5, 5e-5\}, while the batch size is in \{12, 16, 32\} depending on tasks. The maximum length of the input sentence is 384 for SQuAD2.0 and 256/512 for other tasks.  We use AdamW~\cite{loshchilov2018decoupled} as the optimizer, and set the $\beta_2$ and weight decay as 0.98 and 0.01, respectively. All experiments are conducted on NVIDIA A100 GPUs.
The detailed hyper-parameters are provided in Appendix~\ref{appendix_parameters}.

\paragraph{Compared Methods.} For references, we compare our $\mathbb{SE}$ method with other cutting-edge counterparts. Specifically, taking the BERT$\rm_{\texttt{base}}$ as the baseline, we use the following masking strategies to further improve its performance:
\begin{itemize}
    \item Entity-level masking: following~\citet{sun2019ernie}, we mask the named entities in the sentence and enforce the model to predict them.
    \item Span-level masking: as done in~\cite{joshi2020spanbert}, we randomly select spans from the sentence based on a geometric distribution and mask the selected span.
    \item PMI-based masking: similar to~\cite{sadeq2022informask}, we use PMI to identify a set of contiguous (informative) N-grams and mask them.
    \item Self-questioning masking\footnote{The main difference from our full $\mathbb{SE}$ is that it does not involve the self-evolution training process of \textbf{stage 2}.}: We adopt our \textbf{stage 1} to select the hard-to-learn tokens and directly follow the vanilla MLM to mask them and predict the one-hot labels.
\end{itemize}
Notably, for a fair comparison, we implement all these methods in a continual pretraining manner, same to the settings of our $\mathbb{SE}$.

\input{tables/main_results2.tex}
\input{tables/lama.tex}
\input{tables/ablation_metric.tex}

\subsection{Main Results}
\paragraph{$\mathbb{SE}$ surpasses the previous carefully-designed masking strategies.} Results on GLUE and SuperGLUE benchmarks are shown in Table~\ref{tab:main1}. Compared with the baseline BERT$\rm_{\texttt{base}}$, all masking strategies bring the average performance gains, proving the necessity of improving MLM. Among all these methods, our proposed self-questioning masking achieves the relatively better performance on many tasks, confirming the effectiveness of using the PLMs themselves to select the hard-to-learn tokens. More encouragingly, with the help of self-evolution training, our final BERT-SE$\rm_{\texttt{base}}$ can achieve further performance improvements. These results can prove the superiority of our $\mathbb{SE}$.


\paragraph{$\mathbb{SE}$ brings consistent and significant performance improvements among all PLMs.} 
In addition to the results upon BERT$\rm_{\texttt{base}}$, we also apply our method on more discriminative PLMs and report the results in Table~\ref{tab:main1}.
Compared with the baselines, $\mathbb{SE}$ brings consistent and significant performance improvements across all BERT/RoBERTa model sizes. Specifically, for Base and Large RoBERTa models, $\mathbb{SE}$ brings 2.36\% and 2.03\% relative gains in overall score respectively. Also, the gain for BERT is up to 2.24\%. These results prove the effectiveness and universality of our $\mathbb{SE}$.

% \paragraph{SE tends to perform better on stronger PLMs.} Comparing the results of different backbone PLMs, we can observe that the overall gains of $\mathbb{SE}$ method on stronger PLMs are usually higher than those of weaker PLMs, e.g. averaging +1.55\% \textit{vs.} +1.88\% for BERT and RoBERTa. 
% % compared to BERT$\rm_{\texttt{base}}$ (1.18\%), the performance improvements on BERT$\rm_{\texttt{large}}$ (1.92\%) and RoBERTa$\rm_{\texttt{base}}$ (2.03\%) are larger. 
% We attribute this phenomenon to the effect of TLS approach, as the referential probabilities predicted by stronger PLMs contain more linguistic knowledge and are more beneficial for self-evolution training.

\paragraph{$\mathbb{SE}$ enhances the ability of knowledge learning.} For the knowledge-intense tasks, \textit{i.e.}, SQuAD2.0 and SWAG, we report the results in Table~\ref{tab:main2}. With the help of $\mathbb{SE}$, all PLMs consistently achieve better performance. Specifically, the performance improvements on SQuAD2.0 in terms of EM and F1 are up to 0.71\% and 0.64\%, respectively. 
Besides QA tasks that require to be fine-tuned, we conduct experiments on a widely-used factual knowledge probing task, \textit{i.e.}, LAMA~\cite{petroni2019language}, 
to verify whether $\mathbb{SE}$ improves the ability of PLMs on commonsense knowledge.
% we conduct experiments on the widely used knowledge-intense probing task, i.e., LAMA~\cite{petroni2019language}. Specifically, LAMA has around 70,000 factual probing samples across 46 factual relations, providing a set of knowledge sources that are composed of a corpus of facts. 
We report the results in Table~\ref{tab_lama}. Based on the powerful RoBERTa, $\mathbb{SE}$ still brings significant improvements, \textit{i.e.} +3.8 average score, to the knowledge-learning ability of PLMs.
% and the results (See Appendix~\ref{appendix_lama}, Table~\ref{tab_lama}) continue to show that $\mathbb{SE}$ improves the ability of PLMs on commonsense knowledge reasoning effectively. 
% Due to the space limitation, the detailed results are listed in Appendix~\ref{appendix_lama}.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{lse_ablation.pdf}
    \caption{Parameter analysis of $\lambda$ on BERT-SE$\rm_{\texttt{large}}$.}
    \label{fig:ablation2}
\end{figure}

\subsection{Ablation Study}
We evaluate the impact of each component of our $\mathbb{SE}$, including \textit{i}) token-selecting metrics, \textit{ii}) token-specific label smoothing approach, \textit{iii}) coefficient $\lambda$, and \textit{iv}) more $\mathbb{SE}$ iterations.

\paragraph{Impact of Token Selecting Metrics.}
\label{sec_abalation_metric}
As mentioned in \S\ref{sec:se_method}, we introduce several metrics to select the hard-to-learn tokens in the self-questioning stage. Here, we conduct experiments to analyze the impact of different metrics. Specifically, for reference, we compare the ``Correctness-based'' and ``Confidence-based'' metrics\footnote{Our preliminary study shows the non-complementarity between two token-selecting metrics, we compute their vocabulary distribution difference and give evidence at Appendix~\ref{appendix_statistic_analysis}.}
% Notably, we do not verify the effect of using both metrics at the same time, as we found that the tokens selected by ``Correctness-based'' metric already contain most of tokens selected by the other metric (otherwise it is not) in the preliminary experiments. That is, it is relatively redundant and inefficient to select tokens with the combination of both metrics. The detailed analysis is shown in Appendix~\ref{appendix_statistic_analysis}.} 
with a simple alternative, \textit{i.e.}, ``randomly selecting''. Results in Table~\ref{tab_ablation_metric} show that 1) although the ``randomly selecting'' performs worst, it still outperforms the continually trained baseline, showing the effectiveness of the self-evolution training. 2) both our proposed metrics ``Correctness-based'' and ``Confidence-based'' achieve significantly better performance, confirming our claim that learning on informative yet under-explored tokens can strengthen the capability of PLMs and data efficiency. Notably, the correctness-based metric outperforms the confidence-based metric in most cases, thus leaving as our default setting in $\mathbb{SE}$.
% provide less information for further training of PLMs. When using our proposed metrics, $\mathbb{SE}$ brings much larger performance improvements, confirming our claim that learning on informative yet under-explored tokens can strengthen the capacity of PLMs. Notably, the ``Correctness-based'' metric outperforms the other metrics in most scenarios, thus leaving it as the default setting in this work.

\input{tables/ablation_tls.tex}
\paragraph{Impact of Token-specific Label Smoothing.} A key technology in our $\mathbb{SE}$ is the TLS, which uses the token-specific smoothed label to adaptively guide training. To verify its effectiveness, we conduct experiments and present the results in Table~\ref{tab_ablation_tls}. We show that 1) the vanilla label smoothing approach equipped $\mathbb{SE}$ could easily outperform the continuously trained backbone, showing the superiority of our $\mathbb{SE}$ framework, and importantly, 2) our TLS could further improve the results by a large margin against vanilla LS equipped $\mathbb{SE}$, \textit{e.g.} averaging +0.71, indicating the effectiveness of TLS.
% ``-w/o LS'' means that no LS approach is used (directly using the original one-hot labels) and ``-w/ vanilla LS'' refer to using the vanilla LS (a uniform distribution is used to smooth the one-hot labels). Obviously, 
% ``-w/o LS'' performs worst, confirming that 
% directly enforcing the PLMs to fix the one-hot labels would lead to overfitting or over-confidence problems. 
% ``w/ TLS'' (with our TLS approach) outperforms the other counterparts in most settings. These results demonstrate the efficacy of TLS in the self-evolution training stage. 


\paragraph{Impact of Coefficient $\lambda$.} The factor
$\lambda$ in Eq.~\ref{label_smoothing}, which is used to control the ratio of label smoothing, is an important hyper-parameters. In this study, we analyze its influence by evaluating the performance with different $\lambda$ spanning \{0.1, 0.3, 0.5, 0.7, 0.9\} on several GLUE tasks. Figure~\ref{fig:ablation2} illustrates the average results. Compared with the baseline, our $\mathbb{SE}$ consistently brings improvements across all ratios of $\lambda$, basically indicating that the performance of $\mathbb{SE}$ is not sensitive to $\lambda$. More specifically, the case of $\lambda = 0.1$ performs best, and we thereby use this setting in our experiments.
% Then, we sequentially examine the effect of $\mathcal{T}$ by evaluating BERT-$\mathbb{SE}\rm_{\texttt{base}}$ upon different $\mathcal{T}$ (in \{0.05,0.1,0.5,1,5,10\}) on all benchmarks. Table~\ref{tab_ablation_threshold} shows the average results. 

% Here, we evaluate the performance of $\mathbb{SE}$ with different $\lambda$ on GLUE and SuperGLUE to analyze its effect. The overall scores under different $\lambda$ are illustrated in Figure~\ref{fig:ablation2}. Compared to the baseline, our $\mathbb{SE}$ consistently performs better across all ratios of $\lambda$, indicating that $\mathbb{SE}$ is not sensitive to $\lambda$. Despite that, as the ratio increases, the performance of $\mathbb{SE}$ tends to decrease slightly. Thus, we lastly set the $\lambda = 0.1$ in our experiments. 

\input{tables/iterativeSE.tex}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{task_transfer.pdf}
    \caption{\label{fig:task_tranfer}Analysis of task generalization. The model is fine-tuned on the QNLI task and transferred to four different tasks. We can see that $\mathbb{SE}$ consistently brings better generalization compared with its  counterparts.}
    \label{fig:task_transfer}
\end{figure}

\begin{figure*}[ht]
	\centering
	\includegraphics[width=0.89\textwidth]{3d_landscape.pdf} 
	\caption{The 3D loss surface comparison between baseline, $\mathbb{SE}$ (``-w/ vanilla LS'')  and $\mathbb{SE}$ (``-w/ TLS'') methods applied to RoBERTa$\rm_{\texttt{base}}$. Note that the PLMs are fine-tuned on the CoLA task. 
 % It can be seen that $\mathbb{SE}$ methods significantly smooth the loss surface, i.e., improving the model generalization effectively.
	}
	\label{fig:3d_loss}
\end{figure*}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{1d_landscape.pdf}
    \caption{1D visualization of loss landscapes of RoBERTa$\rm_{\texttt{base}}$ models fine-tuned on different tasks. }
    \label{fig:1d_loss}
\end{figure}


\paragraph{Impact of More $\mathbb{SE}$ Iterations.}
Researchers may doubt whether $\mathbb{SE}$ can be further augmented by performing the self-questioning and token-specific label smoothing with already evolved PLMs that own better representations. That is, whether more iterations (denoted as ``$N$'') further enhance $\mathbb{SE}$? 
To answer this question, we continuously train the PLMs with more $\mathbb{SE}$ iterations and report the performance of several GLUE tasks in Table~\ref{tab:iterations}. As seen, increasing the iterations improves the performance but the gain margin is insignificant. Given that increasing $N$ costs more, we suggest using $\mathbb{SE}$ for only one iteration to achieve a better trade-off between costs and performance.

==> [ACL23] SE4PLMs-Camera_Ready/sections/5_discussion.tex <==
\section{Discussion}
\label{sec:discussion}
To better understand $\mathbb{SE}$, we conduct extensive analyses to discuss whether it gains better generalization/ robustness and knowledge-learning ability.

\subsection{Does $\mathbb{SE}$ Bring Better Generalization?}
We examine from two perspectives: \textit{i}) measuring the cross-task zero-shot performance, and \textit{ii}) visualizing the loss landscapes of PLMs.

\paragraph{Task Generalization.} 
The performance of out-of-domain (OOD) data is widely used to verify the model generalization~\cite{Wang2022UnderstandingAI,ding2022redistributing}. Thus, we follow~\citet{xu2021raise,zhong2022improving} and evaluate the performance of PLMs on several OOD data. In practice, we first fine-tune RoBERTa$\rm_{\texttt{base}}$ models trained with different methods (including ``Baseline'', ``$\mathbb{SE}$ (-w/ LS)'', and ``$\mathbb{SE}$ (-w/ TLS)'') on the QNLI task, and then inference on other tasks, \textit{i.e.}, CoLA, MRPC, STS-B, and RTE. The results are illustrated in Figure~\ref{fig:task_transfer}.
We observe that ``$\mathbb{SE}$ (-w/ TLS)'' consistently outperforms the other counterparts. To be more specific, compared with baseline, our $\mathbb{SE}$ brings a +2.90 average improvement score on these tasks, indicating that \textbf{\textit{our $\mathbb{SE}$ boosts the performance of PLMs on OOD data.}}

\paragraph{Visualization of Landscape.} To have a close look, we visualize the loss landscapes of different RoBERTa$\rm_{\texttt{base}}$ models fine-tuned on the CoLA task. In practice, we first show the 3D loss surface results in Figure~\ref{fig:3d_loss} following the ``filter normalized'' setting in~\cite{li2018visualizing,zan2022complementarity}. 
% by sampling 25$\times$25 points in the range of [-1, 1] from random ``filter normalized'' directions, as implemented in~\cite{li2018visualizing}. 
As seen, $\mathbb{SE}$-equipped PLMs show flatter smoother surfaces compared with the vanilla.
To closely compare the differences of ``$\mathbb{SE}$ (-w/ LS)'' and ``$\mathbb{SE}$ (-w/ TLS)'' in the loss landscape, we follow~\citet{he2021effectiveness} to plot the 1D loss curve on more tasks
% \footnote{Additionally, we also follow some prior works~\cite{li2018visualizing,zhong2022improving} and show the 3D loss surface results in Appendix~\ref{appendx_3d} (Figure~\ref{fig:3d_loss}). The 3D visualizations show similar results, i.e., $\mathbb{SE}$ benefits to smooth the loss landscape.}
in Figure~\ref{fig:1d_loss}. We find that through detailed 1D visualization, our optimal setting ``$\mathbb{SE}$ (-w/ TLS)'' shows a flatter and optimal property.
% by linear interpolation between the PLMs weights before (denoted as $\theta_0$) and after (denoted as $\theta_1$) fine-tuning, \textit{i.e.}, ``$\theta_1+\alpha \cdot (\theta_1-\theta_0)$'', where $\alpha$ is a scalar parameter that is ranged from -1 to 1. 
% From both results, we can find that the landscape of RoBERTa-SE$\rm_{\texttt{base}}$ (``-w/ TLS'') has a lower loss and is much flatter than the others. 
\textbf{\textit{These results prove that $\mathbb{SE}$ can smooth the loss landscape and improve the generalization of PLMs effectively.}}

\begin{figure*}[ht]
	\centering
	\includegraphics[width=0.95\textwidth]{cloze_test.pdf} 
	\caption{Cloze test comparison between BERT$\rm_{\texttt{base}}$ and  BERT-SE$\rm_{\texttt{base}}$. The correct predictions are in \textbf{bold}.
	}
	\label{fig:cloze}
\end{figure*}

\subsection{Cloze Test}
To verify whether $\mathbb{SE}$ enforces the PLMs to learn from the informative tokens, we follow~\citet{sun2019ernie} and apply the Cloze test~\cite{taylor1953cloze} to evaluate the knowledge learning ability of PLMs. For each test sample, we first remove the informative token and then enforce the PLMs to infer what it is. Some cases are shown in Figure~\ref{fig:cloze}.

In case 1 and case 2, both BERT$\rm_{\texttt{base}}$ and BERT-SE$\rm_{\texttt{base}}$ can successfully predict the type of masked tokens according to the contexts. However, with the help of the $\mathbb{SE}$ mechanism, BERT-SE$\rm_{\texttt{base}}$ performs more correctly on filling in the slot. Dramatically, in case 3, the baseline BERT$\rm_{\texttt{base}}$ makes unreasonable predictions. One possible reason is that the baseline PLM only learns the shallow pattern and fails to understand the meaning of the context. Additionally, due to the unsatisfactory ability of the baseline PLM on commonsense reasoning, the baseline PLM also predicts strangely in case 4. Different from the baseline, while BERT-SE$\rm_{\texttt{base}}$ does not predict the completely correct tokens in case 3 and case 4, it can capture deep patterns and make more reasonable predictions. \textbf{\textit{In general, these cases prove that $\mathbb{SE}$ indeed improves the knowledge-learning ability of PLMs.}}

\paragraph{\large{\ding{43}} More analyses in Appendix} In addition to the above discussions, we conduct more related analyses and show them in Appendix, \textit{e.g.}, parameter analyses on $\mathcal{T}_l$ and $\mathcal{T}_e$ (Appendix~\ref{appendix_parameter_analysis}), robustness analysis based on the empirical results on AdvGLUE~\cite{wang2021adversarial} (Appendix~\ref{appendix_advglue}), and non-complementarity analysis between token-selecting metrics (Appendix~\ref{appendix_statistic_analysis}). Please refer to Appendix for more details.

==> [ACL23] SE4PLMs-Camera_Ready/sections/6_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
% \textcolor{red}{[DL edited here]}
In this paper, we propose a simple and effective self-evolution ($\mathbb{SE}$) learning mechanism to improve the existing discriminative PLMs by fully exploiting the knowledge from data. $\mathbb{SE}$ follows two stages, \textit{i.e.}, \textit{self-questioning} and \textit{self-evolution training}, and can be used to evolve any MLM-based PLMs with a simple recipe: continue pretraining with $\mathbb{SE}$.
% first adopts a \textit{self-questioning} process to enforce a PLM to wisely locate the informative yet under-explored tokens, and then encourage the PLM to further learn from them in the \textit{self-evolution training} stage. In addition, we introduce a novel token-specific label smoothing approach to adaptively regularize the training.
% Specifically, to alleviate the overfitting problem in the self-evolution training stage, we further propose a novel token-specific label smoothing (TLS) approach to adaptively regularize the training. 
We empirically demonstrated the effectiveness and universality of the $\mathbb{SE}$ on a series of widely-used benchmarks. Further analyses show our approach improves the generalization, robustness, and knowledge-learning ability.
% Experiments show that our $\mathbb{SE}$ brings consistent and significant performance improvements among 4 PLMs. Extensive analyses prove that, with our $\mathbb{SE}$ mechanism, the PLMs can perform better on the knowledge-intense tasks, and have better model generalization and robustness.
% contains two-stage processes: \textit{self-questioning} and \textit{self-evolution training}. In the first stage, we propose two simple model-dependent metrics to leverage the behavior of PLM on individual tokens to select the informative but under-explored tokens. In the self-evolution training stage, to avoid overfitting and over-confidence problems,
% Different from the previous carefully-designed masking strategies that rely on external resource or supervision to select the informative tokens, our self-evolution learning aims to enforce the existing PLMs to wisely predict the informative but under-explored tokens. 
% we further propose a novel token-specific label smoothing (TLS) approach to adaptively regularize the training for each masked token. The TLS approach adopts a smoothing label distribution calibrated with (self-distillation) teacher predictions to supervise the model predictions. 
% We apply the $\mathbb{SE}$ method on 4 PLMs and evaluate their performance on a diverse of 10 tasks, including GLUE, SuperGLUE, SQuAD2.0 and SWAG benchmarks. Experimental results show the effectiveness and universality of SE. Additionally, systematic studies on knowledge-intense tasks prove that $\mathbb{SE}$ can improve the ability of PLMs on knowledge learning. Lastly, we also demonstrate that $\mathbb{SE}$ indeed improves the generalization and robustness of PLMs.
% We reveal that the existing discriminative PLMs can be further improved by fully learning the linguistic knowledge from the pretraining data.
We hope our work could facilitate more research on how to improve existing trained models after all the previous PLM weights are expensive and knowledgeable. 

% For future work, we would like to explore our self-evolution learning mechanism in more scenarios, such as generative PLMs and other downstream tasks. 

\section*{Limitations}
Our work has several potential limitations.
First, given the limited computational budget, we only validate our self-evolution learning on the Large and Base sizes. It will make our work more convincing if scaling the experiments up to the larger model size and training corpus. 
On the other hand, besides the improved commonsense knowledge learning ability, we believe that there are still other abilities, \textit{e.g.}, mathematical word problems, of PLMs that can be improved by our method, which are not fully explored in this work.

\section*{Ethics and Reproducibility Statements}
\paragraph{Ethics} We take ethical considerations very seriously, and strictly adhere to the ACL Ethics Policy. This paper focuses on higher data and model efficiency for discriminative pretrained language models, but not capturing the privacy knowledge. Both the pretraining datasets and models used in this paper are publicly available and have been widely adopted by researchers. Therefore, we believe that this research will not pose ethical issues.

\paragraph{Reproducibility} We will publicly release our code in \url{https://github.com/WHU-ZQH/SE4PLMs} to help reproduce the experimental results of this paper. 

\section*{Acknowledgements}
We are grateful to the anonymous reviewers and the area chair for their insightful comments and suggestions.
This work was supported
%in part by the National Key Research and Development Program of China under Grant 2021YFB2401302, and 
in part by the National Natural Science Foundation of China under Grants 62225113 and 62076186, and in part by the Science and Technology Major Project of Hubei Province (Next-Generation AI Technologies) under Grant 2019AEA170. The numerical calculations in this paper have been done on the supercomputing system in the Supercomputing Center of Wuhan University. 

==> [ACL23] SE4PLMs-Camera_Ready/tables/ablation_metric.tex <==
% \begin{table*}[]
% \centering
% \scalebox{0.9}{
% \begin{tabular}{cccccc}
% \toprule
% \textbf{Method} & \textbf{BERT}$\rm_{\texttt{base}}$             & \textbf{BERT}$\rm_{\texttt{large}}$              & \textbf{RoBERTa}$\rm_{\texttt{base}}$            & \textbf{RoBERTa}$\rm_{\texttt{large}}$   & \textbf{Avg.}     \\
% \midrule
% Baseline                    & 75.97                    & 79.12                    & 78.44                    & 82.35     & \underline{78.97}                 \\ 
% \hdashline
% \multicolumn{6}{l}{Selecting metrics in \textit{self-question} stage}  \\
% \multicolumn{1}{l}{\quad -w/ randomly selecting}  &75.76 (-0.21)   &79.70 (+0.58)   &78.74 (+0.30)   &82.85 (+0.50)  &\underline{79.26 (+0.29)}  \\	
% \multicolumn{1}{l}{\quad -w/ Correctness-based}                                 & 77.15 (+1.18)                              & \textbf{81.04 (+1.92)}                                          & \textbf{80.47 (+2.03)}                                   & \textbf{84.08 (+1.73)}                   & \underline{\textbf{80.69 (+1.72)}}                \\
% \multicolumn{1}{l}{\quad -w/ Confidence-based}                      & \textbf{77.41 (+1.44)}                    & 80.28 (+1.16)                                & 79.43 (+0.98)                                & 83.61 (+1.26)                      & \underline{80.18 (+1.21)}    \\
% \bottomrule
% \end{tabular}
% }
% \caption{Ablation study of different metrics used to select the hard-to-learn tokens in SE, evaluated on the combination of GLUE and SuperGLUE benchmarks. For simplicity, we show the overall score and relative gains in this table. The full results can be found in Table~\ref{tab:all_results}.}
% \label{tab_ablation_metric}
% \end{table*}

\begin{table*}[]
\centering
\scalebox{0.9}{
\begin{tabular}{cccccc}
\toprule
\textbf{Method} & \textbf{BERT}$\rm_{\texttt{base}}$             & \textbf{BERT}$\rm_{\texttt{large}}$              & \textbf{RoBERTa}$\rm_{\texttt{base}}$            & \textbf{RoBERTa}$\rm_{\texttt{large}}$   & \textbf{\underline{Avg.}}     \\
\midrule
Baseline                    & 74.10                    & 77.54                    & 76.73                    & 81.03    & \underline{77.35}                 \\ 
\hdashline
\multicolumn{6}{l}{Selecting metrics in \textit{self-questioning} stage}  \\
\multicolumn{1}{l}{\quad -w/ randomly selecting}  &73.85 (\textcolor{red}{-0.25})   &78.28 (\textcolor[RGB]{0,176,80}{+0.74})   &77.09 (\textcolor[RGB]{0,176,80}{+0.36})   &81.64 (\textcolor[RGB]{0,176,80}{+0.61})  &\underline{77.72 (\textcolor[RGB]{0,176,80}{+0.37})}  \\	
\multicolumn{1}{l}{\quad -w/ Correctness-based}                                 & 75.45 (\textcolor[RGB]{0,176,80}{+1.35})                              & \textbf{79.78 (\textcolor[RGB]{0,176,80}{+2.24)}}                                          & \textbf{79.08 (\textcolor[RGB]{0,176,80}{+2.35)}}                                   & \textbf{83.06 (\textcolor[RGB]{0,176,80}{+2.03)}}                   & \underline{\textbf{79.34 (\textcolor[RGB]{0,176,80}{+1.99)}}}                \\
\multicolumn{1}{l}{\quad -w/ Confidence-based}                      & \textbf{75.77 (\textcolor[RGB]{0,176,80}{+1.67)}}                    & 78.88 (\textcolor[RGB]{0,176,80}{+1.34})                                & 77.86 (\textcolor[RGB]{0,176,80}{+1.13})                                & 82.46 (\textcolor[RGB]{0,176,80}{+1.43})                      & \underline{78.74 (\textcolor[RGB]{0,176,80}{+1.39)}}    \\
\bottomrule
\end{tabular}
}
\caption{Ablation study of different metrics used to select the hard-to-learn tokens in $\mathbb{SE}$, evaluated on the combination of GLUE and SuperGLUE benchmarks. For simplicity, we show the overall score here. The full results and analyses about the superiority of the correctness-based metric can be found in Appendix (Table~\ref{tab:all_results}\&\ref{tab:statistic}).}
\label{tab_ablation_metric}
\end{table*}

==> [ACL23] SE4PLMs-Camera_Ready/tables/ablation_threshold.tex <==
% \begin{table}[t]
% \centering
% \scalebox{0.85}{
% \begin{tabular}{lcc}
% \toprule
% \multirow{2}{*}{Method} & GLUE/SGLUE & SQuAD2.0/SWAG \\ \cmidrule{2-3}
% \multicolumn{1}{c}{} & \textit{Avg. ($\Delta$)} & \textit{Avg. ($\Delta$)} \\ \midrule \midrule
% BERT$\rm_{\texttt{base}}$ & 75.97 & 74.93 \\ \hdashline
% \multicolumn{3}{l}{BERT-SE$\rm_{\texttt{base}}$} \\
% \quad $\mathcal{T}=0.05$ & 76.44 (+0.47) & 75.44 (+0.51) \\
% \quad $\mathcal{T}=0.1$ & \textbf{77.15 (+1.18)} & \textbf{75.48 (+0.55)} \\
% \quad $\mathcal{T}=0.5$ & 75.81 (-0.16) & 75.22 (+0.29) \\
% \quad $\mathcal{T}=1$ & 75.85 (-0.12) & 75.37 (+0.44) \\
% \quad $\mathcal{T}=5$ & 75.39 (-0.58) & 75.05 (+0.12) \\
% \quad $\mathcal{T}=10$ & 75.05 (-0.95) & 74.82 (-0.11) \\
% \bottomrule
% \end{tabular}
% }
% \caption{Parameter analysis on the threshold $\mathcal{T}$ used in self-questioning stage. The ``Correctness-based'' metric is used in this study. Full results are in Table~\ref{tab:all_results2}.}
% \label{tab_ablation_threshold}
% \end{table}

\begin{table}[t]
\centering
\scalebox{0.85}{
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{Method} & GLUE/SGLUE & SQuAD2.0/SWAG \\ \cmidrule{2-3}
\multicolumn{1}{c}{} & \textit{Avg. ($\Delta$)} & \textit{Avg. ($\Delta$)} \\ \midrule \midrule
BERT$\rm_{\texttt{base}}$ & 74.10 & 74.93 \\ \hdashline
\multicolumn{3}{l}{BERT-SE$\rm_{\texttt{base}}$} \\
\quad $\mathcal{T}_l=0.05$ & 74.63 (\textcolor[RGB]{0,176,80}{+0.53}) & 75.44 (\textcolor[RGB]{0,176,80}{+0.51}) \\
\quad $\mathcal{T}_l=0.1$ & \textbf{75.45 (\textcolor[RGB]{0,176,80}{+1.35})} & \textbf{75.48 (\textcolor[RGB]{0,176,80}{+0.55})} \\
\quad $\mathcal{T}_l=0.5$ & 73.93 (\textcolor{red}{-0.17}) & 75.22 (\textcolor[RGB]{0,176,80}{+0.29}) \\
\quad $\mathcal{T}_l=1$ & 74.02 (\textcolor{red}{-0.08}) & 75.37 (\textcolor[RGB]{0,176,80}{+0.44}) \\
% \quad $\mathcal{T}_l=5$ & 73.47 (-0.63) & 75.05 (+0.12) \\
% \quad $\mathcal{T}_l=10$ & 73.08 (-1.02) & 74.82 (-0.11) \\
\bottomrule
\end{tabular}
}
\caption{Parameter analysis on the threshold $\mathcal{T}_l$ used in self-questioning stage. The ``Correctness-based'' metric is used in this study. Full results are in Table~\ref{tab:all_results2}.}
\label{tab_ablation_threshold}
\end{table}

==> [ACL23] SE4PLMs-Camera_Ready/tables/ablation_tls.tex <==
% \begin{table}[t]
% \centering
% \scalebox{0.85}{
% \begin{tabular}{lcc}
% \toprule
% \multirow{2}{*}{\bf Method} &\bf GLUE/SGLUE &\bf SQuAD/SWAG \\ \cmidrule{2-3}
% \multicolumn{1}{c}{} & \textit{Avg. ($\Delta$)} & \textit{Avg. ($\Delta$)} \\ \midrule
% RoBERTa$\rm_{\texttt{base}}$ & 78.44 & 80.13 \\ \hdashline
% \multicolumn{3}{l}{RoBERTa-SE$\rm_{\texttt{base}}$} \\
% \quad -w/o LS & 80.07 (+1.63) & 80.04 (-0.09) \\
% \quad -w/ vanilla LS & 80.16 (+1.72) & 80.37 (+0.24) \\
% \quad -w/ TLS (Ours) & \textbf{80.47 (+2.03)} & \textbf{80.61 (+0.48)} \\
% \bottomrule
% \end{tabular}
% }
% \caption{Analysis on the TLS approach used in our SE. Notably, ``-w/o LS'' means that no LS approach is used and ``-w/ pure LS'' refer to using the vanilla LS approach in SE mechanism. Full results are shown in Table~\ref{tab:all_results2}.}
% \label{tab_ablation_tls}
% \end{table}

%updated results after removing the STS-B
\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{\bf Method} &\bf GLUE/SGLUE &\bf SQuAD/SWAG \\ \cmidrule{2-3}
\multicolumn{1}{c}{} & \textit{Avg. ($\Delta \uparrow$)} & \textit{Avg. ($\Delta \uparrow$)} \\ \midrule
RoBERTa$\rm_{\texttt{base}}$ & 76.73 & 80.13 \\ \hdashline
\multicolumn{3}{l}{RoBERTa-SE$\rm_{\texttt{base}}$} \\
% \quad -w/o LS & 78.61 (+1.88) & 80.04 (-0.09) \\
\quad -w/ vanilla LS & 78.37 (\textcolor[RGB]{0,176,80}{+1.64}) & 80.37 (\textcolor[RGB]{0,176,80}{+0.24}) \\
\quad -w/ TLS (Ours) & \textbf{79.08 (\textcolor[RGB]{0,176,80}{+2.35})} & \textbf{80.61 (\textcolor[RGB]{0,176,80}{+0.48})} \\
\bottomrule
\end{tabular}
}
\caption{Ablation study of our TLS approach. ``-w/ vanilla LS'' and ``-w/ TLS (Ours)'' refer to using the vanilla and our proposed token-specific label smoothing approaches in $\mathbb{SE}$ mechanism, respectively. Full results are shown in Appendix (Table~\ref{tab:all_results2}).}
\label{tab_ablation_tls}
\end{table}

==> [ACL23] SE4PLMs-Camera_Ready/tables/advglue.tex <==
% \begin{table*}[]
%     \center
%     \begin{tabular}{lcccccccc}
% \toprule
%     \multicolumn{1}{c}{\multirow{2}{*}{Method}} & RTE           & SST-2         & QNLI          & \multicolumn{2}{c}{MNLI} & \multicolumn{2}{c}{QQP}       & \multirow{2}{*}{Avg.} \\
%     \multicolumn{1}{c}{}                        & Acc.          & Acc.          & Acc.          & m-     & mm-             & Acc.          & F1.           &                       \\
%     \midrule \midrule
%     \multicolumn{9}{c}{\cellcolor{lightgray}{\textit{\textbf{Results on BERT-base}}}}                                                                                                                             \\
%     BERT-base-hard                              & \textbf{35.8} & 29.1          & 37.8          & 33.9   & 21.6            & 46.2          & 43.2          & 35.4                  \\
%     BERT-base-hard-sl                           & 34.6          & \textbf{29.7} & 37.2          & 33.1   & \textbf{24.1}   & 46.2          & 41.7          & 35.2                  \\
%     BERT-base-entropy                           & \textbf{35.8} & 28.4          & 34.5          & 32.2   & 22.2            & 44.9          & 41.1          & 34.2                  \\
%     BERT-base-entropy-sl                        & 33.3          & 28.4          & \textbf{42.6} & 33.9   & 23.5            & \textbf{50.0} & \textbf{48.0} & \textbf{37.1}         \\
%     \multicolumn{9}{c}{\cellcolor{lightgray}{\textit{\textbf{Results on BERT-large}}}}                                                                                                                             \\
%     BERT-large-hard                             & 50.6          & 37.8          & 45.9          & 35.5   & 23.5            & 34.6          & 30.1          & 36.9                  \\
%     BERT-large-hard-sl                          & \textbf{53.1} & 35.1          & 45.3          & 34.7   & 24.7            & 37.2          & 34.7          & 37.8                  \\
%     BERT-large-entropy                          & 46.9          & 34.5          & 47.3          & 35.5   & 24.1            & 39.7          & \textbf{39.0} & 38.1                  \\
%     BERT-large-entropy-sl                       & 51.9          & 36.5          & \textbf{52.7} & 35.5   & 24.1            & \textbf{42.3} & 34.8          & \textbf{39.7}        
% \\ \bottomrule    
% \end{tabular}
% \end{table*}

\begin{table*}[t]
\centering
\small
% \scalebox{0.93}
{
    \begin{tabular}{lcccccccccccc}
    \toprule
    \multirow{2}{*}{\bf Method} & \multicolumn{6}{c}{BERT$\rm_{\texttt{base}}$} & 
    \multicolumn{6}{c}{\textsc{RoBERTa}$\rm_{\texttt{base}}$} \\
    \cmidrule(lr){2-7} \cmidrule(lr){8-13}
    ~ & RTE &SST-2 & QNLI & MNLI & QQP & \underline{Avg.} & RTE &SST-2 & QNLI & MNLI & QQP & \underline{Avg.} \\
    \midrule
    % Baseline & 32.1 & \textbf{29.7} & 39.9 & 22.2 & 37.2 & \underline{32.2} & 46.8 & \textbf{41.9} & \textbf{36.5} & 21.6 & 28.2 & \underline{35.0} \\
    Baseline & 32.8 & \textbf{29.7} & 40.5 & 22.8 & 38.5 & \underline{32.9} & \textbf{47.1} & \textbf{41.9} & \textbf{36.2} & 21.0 & 30.9 & \underline{35.4} \\
    % -w/ \textbf{SSE} & \textbf{35.8} & 29.1 & 37.8 & 21.6 & 39.7 & \underline{32.8} & \textbf{49.4} & 39.9 & 33.8 & 22.2 & 32.1 & \underline{35.5} \\
    \textbf{\quad -w/ SE} & \textbf{33.3} & 28.4 & \textbf{42.6} & \textbf{23.5} & \textbf{42.3} & \underline{\textbf{34.0}} & 45.7 & 37.8 & 32.4 & \textbf{23.5} & \textbf{38.5} & \underline{\textbf{35.6}} \\
    \midrule
    \multirow{2}{*}{\bf Method} & \multicolumn{6}{c}{BERT$\rm_{\texttt{large}}$} & 
    \multicolumn{6}{c}{\textsc{RoBERTa}$\rm_{\texttt{large}}$} \\
    \cmidrule(lr){2-7} \cmidrule(lr){8-13}
    ~ & RTE &SST-2 & QNLI & MNLI & QQP & \underline{Avg.} & RTE &SST-2 & QNLI & MNLI & QQP & \underline{Avg.} \\
    \midrule
    % Baseline & 43.2 & 32.4 & 37.2 & 22.8 & 41.0 & \underline{35.3} & 66.5 & 44.1 & \textbf{63.5} & 33.3 & 38.5 & \underline{49.2} \\
    Baseline & 45.6 & \textbf{35.8} & 41.4 & \textbf{25.3} & 45.4 & \underline{38.7} & 64.1 & 43.9 & \textbf{61.5} & 33.9 & 44.9 & \underline{49.7} \\
    % -w/ \textbf{SSE} & 50.6 & \textbf{37.8} & \textbf{45.9} & 23.5 & 46.2& \underline{40.8} & \textbf{67.9} & 46.6 & 57.4 & \textbf{37.0} & 51.3 & \underline{52.0} \\
    \textbf{\quad -w/ SE} & \textbf{53.1} & 35.1 & \textbf{45.3} & 24.7 & \textbf{50.0} & \underline{\textbf{41.6}} & \textbf{67.9} & \textbf{48.6} &58.1 & \textbf{34.6} & \textbf{55.1} & \underline{\textbf{52.9}} \\
    \bottomrule
    \end{tabular}
}
\caption{Comparison between $\mathbb{SE}$ and vanilla method applied to all PLMs on AdvGLUE~\cite{wang2021adversarial} benchmark. Average scores on all tasks are \underline{underlined}. The best results are given in \textbf{bold}. 
% It shows that SE method yields consistent improvements among different PLMs, indicating that SE improves the robustness of PLMs.
}
\label{tab:advglue}
\end{table*}

==> [ACL23] SE4PLMs-Camera_Ready/tables/all_results.tex <==
% \begin{table*}[]
% \centering
% \small
% % \scalebox{0.95}
% {
%     \begin{tabular}{lcccccccccc}
%     \toprule
%     \multicolumn{1}{c}{}                         & CoLA                        & MRPC                        & STS-B                       & RTE                         & BoolQ         & CB            & WiC           & COPA          & \multicolumn{2}{c}{Score}      \\
%     \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-11} 
%     \multicolumn{1}{l}{\multirow{-2}{*}{Method}} & \textit{Mcc.}               & \textit{Acc.}               & \textit{Pear.}              & \textit{Acc.}               & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \textit{\underline{Avg.}} & \textit{$\Delta$} \\
%     \midrule \midrule
%     \multicolumn{11}{l}{{\textbf{\textit{Baseline PLMs}}}}  \\
%     \quad BERT$\rm_{\texttt{base}}$                                & 62.33                        & 88.97                        & 89.04                       & 76.89                        & 75.05          & 85.71          & 66.77          & 63.00          & \underline{75.97}          & -- \\
%     \quad BERT$\rm_{\texttt{large}}$                               & 63.00                        & 87.25                        & 90.20                        & 83.80                        & 78.40          & 91.07         & 67.24          & 72.00          & \underline{79.12}          & --              \\
%     \hdashline
%     \quad RoBERTa$\rm_{\texttt{base}}$                            & 62.00                        & 90.20                        & 90.45                        & 83.12                        & 78.72          & 83.93          & 69.12          & 70.00          & \underline{78.44}          & --              \\
%     \quad RoBERTa$\rm_{\texttt{large}}$                            & 64.73                        & 90.69                        & 91.62                        & 88.44                        & 84.37          & 91.07          & 69.90          & 78.00          & \underline{82.35}          & --              \\ \midrule
%     \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{``\textbf{Randomly selecting}''}}}  \\
%     BERT-SE$\rm_{\texttt{base}}$            &63.23 & 87.01 & 89.12 & 76.17 & 74.83 & 85.70 & 68.00 & 62.00 & \underline{75.76} & -0.21    \\
%     % \hdashline
%     BERT-SE$\rm_{\texttt{large}}$                              & 65.28 & 87.74 & 89.68 & 84.12 & 80.10 & 92.90 & 68.8 & 69.00 & \underline{79.70} & \textcolor[RGB]{0,176,80}{+0.58  \\
%     \hdashline
%     RoBERTa-SE$\rm_{\texttt{base}}$                            & 63.78 & 88.73 & 90.30 & 81.59 & 78.83 & 89.29 & 69.43 & 68.00 & 78.74 & \textcolor[RGB]{0,176,80}{+0.30            \\
%     RoBERTa-SE$\rm_{\texttt{large}}$      & 63.42 & 90.20 & 91.31 & 89.89 & 84.13 & 92.86 & 71.00 & 80.00 & \underline{82.85} & \textcolor[RGB]{0,176,80}{+0.50          \\
%     \midrule
%     \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{``\textbf{Correctness-based}'' metric}}}  \\
%     BERT-SE$\rm_{\texttt{base}}$                         & 63.63 & 89.50 & 89.03 & 77.98 & 74.37 & 89.29 & 67.40 & 66.00 & \underline{77.15} & \textcolor[RGB]{0,176,80}{+1.18            \\
%     BERT-SE$\rm_{\texttt{large}}$                           & 65.66               & 88.23                        & 89.84                        & 85.20               & 80.18          & 92.86          & 68.34          & 78.00          & \underline{81.04}          & \textcolor[RGB]{0,176,80}{+1.92            \\
%     \hdashline
%     RoBERTa-SE$\rm_{\texttt{base}}$                         & 62.11                        & 89.71                       & 90.19                        & 84.12               & 79.39          & 92.86          & 71.40          & 74.00          & \underline{80.47}          & \textcolor[RGB]{0,176,80}{+2.03            \\
%     RoBERTa-SE$\rm_{\texttt{large}}$                       & 67.80               & 91.91               & 91.20                        & 90.25                        & 84.56          & 96.40          & 70.53          & 80.00          & \underline{84.08}          & \textcolor[RGB]{0,176,80}{+1.73            \\
%     \midrule
%     \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{``\textbf{Confidence-based}'' metric}}}  \\ 
%     BERT-SE$\rm_{\texttt{base}}$                         & 63.17                        & 89.22                        & 88.83                        & 80.51               & 73.98          & 89.29          & 67.24          & 67.00          & \underline{77.41}          & \textcolor[RGB]{0,176,80}{+1.44            \\

%     BERT-SE$\rm_{\texttt{large}}$        & 64.07 & 88.48 & 90.12 & 84.84 & 79.30 & 92.86 & 69.59 & 73.00 & \underline{80.28} & \textcolor[RGB]{0,176,80}{+1.16            \\
%     \hdashline
%     RoBERTa-SE$\rm_{\texttt{base}}$                         & 64.06 & 89.71 & 90.35 & 83.03 & 78.10 & 85.71 & 69.44 & 75.00 & \underline{79.43} & \textcolor[RGB]{0,176,80}{+0.98            \\
%     RoBERTa-SE$\rm_{\texttt{large}}$                       & 64.17 & 89.71 & 91.66 & 90.61 & 84.13 & 96.40 & 70.22 & 82.00 & \underline{83.61} & \textcolor[RGB]{0,176,80}{+1.26            \\
%     \bottomrule
% \end{tabular}
% }
% \caption{Full contrastive results (corresponding to the average results in Table~\ref{tab_ablation_metric}) between different metrics used to select the hard-to-learn tokens on the combination of GLUE and SuperGLUE benchmarks. ``$\Delta$'' denotes the improvement of SE methods compared to the baseline PLMs. Average scores on all tasks are \underline{underlined}.}
% \label{tab:all_results}
% \end{table*}

%remove the results of STS-B
\begin{table*}[]
\centering
\small
% \scalebox{0.95}
{
    \begin{tabular}{lcccccccccc}
    \toprule
    \multicolumn{1}{c}{}                         & \bf CoLA                        &\bf  MRPC                                               &\bf  RTE                         & \bf BoolQ         & \bf CB            &\bf  WiC           & \bf COPA          & \multicolumn{2}{c}{\bf Score}      \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-8} \cmidrule(lr){9-10} 
    \multicolumn{1}{l}{\multirow{-2}{*}{\bf Method}} & \textit{Mcc.}               & \textit{Acc.}                             & \textit{Acc.}               & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \textit{\underline{Avg.}} & \textit{$\Delta$} \\
    \midrule \midrule
    \multicolumn{10}{l}{{\textbf{\textit{Baseline PLMs}}}}  \\
    \quad BERT$\rm_{\texttt{base}}$                                & 62.33                        & 88.97                                               & 76.89                        & 75.05          & 85.71          & 66.77          & 63.00          & \underline{74.10}          & -- \\
    \quad BERT$\rm_{\texttt{large}}$                               & 63.00                        & 87.25                                                & 83.80                        & 78.40          & 91.07         & 67.24          & 72.00          & \underline{77.54}          & --              \\
    \hdashline
    \quad RoBERTa$\rm_{\texttt{base}}$                            & 62.00                        & 90.20                                                & 83.12                        & 78.72          & 83.93          & 69.12          & 70.00          & \underline{76.73}          & --              \\
    \quad RoBERTa$\rm_{\texttt{large}}$                            & 64.73                        & 90.69                                                & 88.44                        & 84.37          & 91.07          & 69.90          & 78.00          & \underline{81.03}          & --              \\ \midrule
    \multicolumn{10}{c}{\cellcolor{lightgray}{\textit{``\textbf{Randomly selecting}''}}}  \\
    BERT-SE$\rm_{\texttt{base}}$            &63.23 & 87.01 & 76.17 & 74.83 & 85.70 & 68.00 & 62.00 & \underline{73.85} & \textcolor{red}{-0.25}    \\
    % \hdashline
    BERT-SE$\rm_{\texttt{large}}$                              & 65.28 & 87.74 & 84.12 & 80.10 & 92.90 & 68.8 & 69.00 & \underline{78.28} & \textcolor[RGB]{0,176,80}{+0.74}  \\
    \hdashline
    RoBERTa-SE$\rm_{\texttt{base}}$                            & 63.78 & 88.73 & 81.59 & 78.83 & 89.29 & 69.43 & 68.00 & \underline{77.09} & \textcolor[RGB]{0,176,80}{+0.36}            \\
    RoBERTa-SE$\rm_{\texttt{large}}$      & 63.42 & 90.20 & 89.89 & 84.13 & 92.86 & 71.00 & 80.00 & \underline{81.64} & \textcolor[RGB]{0,176,80}{+0.61}          \\
    \midrule
    \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{``\textbf{Correctness-based}'' metric}}}  \\
    BERT-SE$\rm_{\texttt{base}}$                         & 63.63 & 89.50 & 77.98 & 74.37 & 89.29 & 67.40 & 66.00 & \underline{75.45} & \textcolor[RGB]{0,176,80}{+1.35}            \\
    BERT-SE$\rm_{\texttt{large}}$                           & 65.66               & 88.23                                               & 85.20               & 80.18          & 92.86          & 68.34          & 78.00          & \underline{79.78}          & \textcolor[RGB]{0,176,80}{+2.24}            \\
    \hdashline
    RoBERTa-SE$\rm_{\texttt{base}}$                         & 62.11                        & 89.71                                             & 84.12               & 79.39          & 92.86          & 71.40          & 74.00          & \underline{79.08}          & \textcolor[RGB]{0,176,80}{+2.35}            \\
    RoBERTa-SE$\rm_{\texttt{large}}$                       & 67.80               & 91.91                                     & 90.25                        & 84.56          & 96.40          & 70.53          & 80.00          & \underline{83.06}          & \textcolor[RGB]{0,176,80}{+2.03}            \\
    \midrule
    \multicolumn{10}{c}{\cellcolor{lightgray}{\textit{``\textbf{Confidence-based}'' metric}}}  \\ 
    BERT-SE$\rm_{\texttt{base}}$                         & 63.17                        & 89.22                                              & 80.51               & 73.98          & 89.29          & 67.24          & 67.00          & \underline{75.77}          & \textcolor[RGB]{0,176,80}{+1.67}            \\

    BERT-SE$\rm_{\texttt{large}}$        & 64.07 & 88.48 & 84.84 & 79.30 & 92.86 & 69.59 & 73.00 & \underline{78.88} & \textcolor[RGB]{0,176,80}{+1.34}            \\
    \hdashline
    RoBERTa-SE$\rm_{\texttt{base}}$                         & 64.06 & 89.71 & 83.03 & 78.10 & 85.71 & 69.44 & 75.00 & \underline{77.86} & \textcolor[RGB]{0,176,80}{+1.13}            \\
    RoBERTa-SE$\rm_{\texttt{large}}$                       & 64.17 & 89.71 & 90.61 & 84.13 & 96.40 & 70.22 & 82.00 & \underline{82.46} & \textcolor[RGB]{0,176,80}{+1.43}           \\
    \bottomrule
\end{tabular}
}
\caption{Full comparison results (corresponding to the average results in Table~\ref{tab_ablation_metric}) between different metrics used to select the hard-to-learn tokens on the combination of GLUE and SuperGLUE benchmarks. ``$\Delta$'' denotes the improvement of $\mathbb{SE}$ methods compared to the baseline PLMs. Average scores on all tasks are \underline{underlined}.}
\label{tab:all_results}
\end{table*}

% \begin{table*}[]
% \centering
% \small
% % \scalebox{0.85}
% {
%     \begin{tabular}{lccccccccccc}
%     \toprule
%     \multicolumn{1}{c}{}                         & CoLA                        & MRPC                        & STS-B                       & RTE                         & BoolQ         & CB            & WiC           & COPA          & \multicolumn{2}{c}{SQuAD2.0}  &SWAG    \\
%     \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-12} 
%     \multicolumn{1}{l}{\multirow{-2}{*}{Method}} & \textit{Mcc.}               & \textit{Acc.}               & \textit{Pear.}              & \textit{Acc.}               & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \textit{EM} & \textit{F1} &\textit{Acc.} \\
%     \midrule 
%     RoBERTa$\rm_{\texttt{base}}$                            & 62.00                        & \textbf{90.20}                        & 90.45                        & 83.12                        & 78.72          & 83.93          & 69.12          & 70.00          & 78.79          & 81.92 &79.69              \\
%     \hdashline
%     \multicolumn{12}{l}{RoBERTa-SE$\rm_{\texttt{base}}$} \\   
%     \quad -w/o LS &\textbf{64.18} & 88.48 & 90.29 & 83.39 & 78.89 & 89.29 & \textbf{73.04} & 73.00 & 78.64 & 81.75 &79.72 \\
%     \quad -w/ pure LS &63.18 & 89.71 & \textbf{92.68} & 83.39 & 78.29 & 89.29 & 69.75 & \textbf{75.00} & 79.01 &82.12 &79.97 \\
%     \quad -w/ TLS (Ours) & 62.11                        & 89.71                       & 90.19                        & \textbf{84.12}               & \textbf{79.39}          & \textbf{92.86}          & 71.40          & 74.00          & \textbf{79.41}         & \textbf{82.55} &\textbf{79.88}            \\  
%     \bottomrule
%     \toprule
%     BERT$\rm_{\texttt{base}}$  &62.33 & 88.97 & 89.04 & 76.89 & \textbf{75.05} & 85.71 & 66.77 & 63.00 & 72.85 & 75.63 & 77.83 \\
%     \hdashline
%     \multicolumn{12}{l}{BERT-SE$\rm_{\texttt{base}}$} \\
%     \quad $\mathcal{T}=0.05$ &63.30 & 87.50 & \textbf{89.10} & 77.26 & 73.91 & 85.71 & 67.71 & \textbf{67.00} & 72.85 & 75.63 & 77.83 \\
%     \quad $\mathcal{T}=0.1$ &\textbf{63.63} & \textbf{89.50} & 89.03 & \textbf{77.98} & 74.37 & \textbf{89.29} & 67.40 & 66.00 & \textbf{72.89} & \textbf{75.64} & \textbf{77.91} \\
%     \quad $\mathcal{T}=0.5$ &61.31 & 88.24 & 88.99 & 77.26 & 73.88 & 85.71 & 67.08 & 64.00 & 72.46 & 75.36 & 77.84 \\
%     \quad $\mathcal{T}=1$ &62.06 & 88.24 & 88.65 & 77.26 & 73.82 & 82.14 & 68.65 & 66.00 & 72.62 & 75.56 & 77.93 \\
%     \quad $\mathcal{T}=5$ &62.00 & 87.99 & 88.84 & 76.90 & 73.85 & 82.14 & \textbf{69.43} & 62.00 & 72.33 & 75.28 & 77.53 \\
%     \quad $\mathcal{T}=10$ &61.06 & 87.99 & 88.58 & 77.26 & 73.73 & 80.36 & 68.18 & 63.00 & 72.13 & 74.97 & 77.37 \\
%     \bottomrule
% \end{tabular}
% }
% \caption{Full contrastive results (corresponding to the average results in Table~\ref{tab_ablation_tls} and~\ref{tab_ablation_threshold}, respectively) on the combination of GLUE, SuperGLUE, SQuAD2.0 and SWAG benchmarks. Best results are in \textbf{bold}.}
% \label{tab:all_results2}
% \end{table*}



\begin{table*}[]
\centering
\small
% \scalebox{0.85}
{
    \begin{tabular}{lcccccccccc}
    \toprule
    \multicolumn{1}{c}{}                         & CoLA                        & MRPC                                               & RTE                         & BoolQ         & CB            & WiC           & COPA          & \multicolumn{2}{c}{SQuAD2.0}  &SWAG    \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-8} \cmidrule(lr){9-11} 
    \multicolumn{1}{l}{\multirow{-2}{*}{Method}} & \textit{Mcc.}               & \textit{Acc.}              & \textit{Acc.}               & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \textit{EM} & \textit{F1} &\textit{Acc.} \\
    \midrule 
    RoBERTa$\rm_{\texttt{base}}$                            & 62.00                        & \textbf{90.20}                                                & 83.12                        & 78.72          & 83.93          & 69.12          & 70.00          & 78.79          & 81.92 &79.69              \\
    \hdashline
    \multicolumn{11}{l}{RoBERTa-SE$\rm_{\texttt{base}}$} \\   
    % \quad -w/o LS &\textbf{64.18} & 88.48 & 83.39 & 78.89 & 89.29 & \textbf{73.04} & 73.00 & 78.64 & 81.75 &79.72 \\
    \quad -w/ vanilla LS &63.18 & 89.71 & 83.39 & 78.29 & 89.29 & 69.75 & \textbf{75.00} & 79.01 &82.12 &79.97 \\
    \quad -w/ TLS (Ours) & 62.11                        & 89.71                                         & \textbf{84.12}               & \textbf{79.39}          & \textbf{92.86}          & 71.40          & 74.00          & \textbf{79.41}         & \textbf{82.55} &\textbf{79.88}            \\  
    % \bottomrule
    \toprule
    BERT$\rm_{\texttt{base}}$  &62.33 & 88.97 & 76.89 & \textbf{75.05} & 85.71 & 66.77 & 63.00 & 72.85 & 75.63 & 77.83 \\
    \hdashline
    \multicolumn{11}{l}{BERT-SE$\rm_{\texttt{base}}$} \\
    \quad $\mathcal{T}_l=0.05$ &63.30 & 87.50 & 77.26 & 73.91 & 85.71 & 67.71 & \textbf{67.00} & 72.85 & 75.63 & 77.83 \\
    \quad $\mathcal{T}_l=0.1$ &\textbf{63.63} & \textbf{89.50} & \textbf{77.98} & 74.37 & \textbf{89.29} & 67.40 & 66.00 & \textbf{72.89} & \textbf{75.64} & \textbf{77.91} \\
    \quad $\mathcal{T}_l=0.5$ &61.31 & 88.24 & 77.26 & 73.88 & 85.71 & 67.08 & 64.00 & 72.46 & 75.36 & 77.84 \\
    \quad $\mathcal{T}_l=1$ &62.06 & 88.24 & 77.26 & 73.82 & 82.14 & 68.65 & 66.00 & 72.62 & 75.56 & 77.93 \\
    % \quad $\mathcal{T}=5$ &62.00 & 87.99 & 88.84 & 76.90 & 73.85 & 82.14 & \textbf{69.43} & 62.00 & 72.33 & 75.28 & 77.53 \\
    % \quad $\mathcal{T}=10$ &61.06 & 87.99 & 88.58 & 77.26 & 73.73 & 80.36 & 68.18 & 63.00 & 72.13 & 74.97 & 77.37 \\
    \bottomrule
\end{tabular}
}
\caption{Full comparison results (corresponding to the average results in Table~\ref{tab_ablation_tls} and~\ref{tab_ablation_threshold}, respectively) on the combination of GLUE, SuperGLUE, SQuAD2.0 and SWAG benchmarks. Best results are given in \textbf{bold}.}
\label{tab:all_results2}
\end{table*}

==> [ACL23] SE4PLMs-Camera_Ready/tables/all_results2.tex <==
% Please add the following required packages to your document preamble:
\begin{table*}[]
\centering
\scalebox{0.85}{
    \begin{tabular}{lcccccccccc}
    \toprule
    \multicolumn{1}{c}{}                         & CoLA                        & MRPC                        & STS-B                       & RTE                         & BoolQ         & CB            & WiC           & COPA          & \multicolumn{2}{c}{Score}      \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-11} 
    \multicolumn{1}{l}{\multirow{-2}{*}{Method}} & \textit{Mcc.}               & \textit{Acc.}               & \textit{Pear.}              & \textit{Acc.}               & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \textit{\underline{Avg.}} & \textit{$\Delta$} \\
    \midrule \midrule
    \multicolumn{11}{l}{{\textbf{\textit{Baseline PLMs}}}}  \\
    \quad BERT$\rm_{\texttt{base}}$                                & 62.33                        & 88.97                        & 89.04                       & 76.89                        & 75.05          & 85.71          & 66.77          & 63.00          & \underline{75.97}          & -- \\
    \quad BERT$\rm_{\texttt{large}}$                               & 63.00                        & 87.25                        & 90.20                        & 83.80                        & 78.40          & 91.07         & 67.24          & 72.00          & \underline{79.12}          & --              \\
    \quad RoBERTa$\rm_{\texttt{base}}$                            & 62.00                        & 90.20                        & 90.45                        & 83.12                        & 78.72          & 83.93          & 69.12          & 70.00          & \underline{78.44}          & --              \\
    \quad RoBERTa$\rm_{\texttt{large}}$                            & 64.73                        & 90.69                        & 91.62                        & 88.44                        & 84.37          & 91.07          & 69.90          & 78.00          & \underline{82.35}          & --              \\ \midrule
    \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{BERT, ``\textbf{loss-based}'' metric}}}  \\
    BERT-SE$\rm_{\texttt{base}}$ (-w/o LS)                            & \textbf{64.78} & 87.99 & \textbf{89.08} & \textbf{78.34} & 74.13 & 85.71 & \textbf{67.87} & \textbf{68.00} & \underline{76.99} & +1.02            \\
    BERT-SE$\rm_{\texttt{base}}$ (-w/ LS)                         & 63.63 & \textbf{89.50} & 89.03 & 77.98 & \textbf{74.37} & \textbf{89.29} & 67.40 & 66.00 & \textbf{\underline{77.15}} & \textbf{+1.18}            \\
    \hdashline
    BERT-SE$\rm_{\texttt{large}}$ (-w/o LS)                              & 64.14                        & \textbf{88.73}               & \textbf{89.95}               & 84.83                        & 79.93          & \textbf{92.86}          & 68.18          & 71.00          & \underline{79.95}          & +0.83            \\
    BERT-SE$\rm_{\texttt{large}}$ (-w/ LS)                           & \textbf{65.66}               & 88.23                        & 89.84                        & \textbf{85.20}               & \textbf{80.18}          & \textbf{92.86}          & \textbf{68.34}          & \textbf{78.00}          & \textbf{\underline{81.04}}          & \textbf{+1.92}            \\
    \midrule
    \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{BERT, ``\textbf{entropy-based}'' metric}}}  \\ 

    BERT-SE$\rm_{\texttt{base}}$ (-w/o LS)                            & 62.82                        & 88.24                        & \textbf{88.86}                        & 77.98                        & 73.43          & 87.50          & \textbf{68.03}          & \textbf{68.00}          & \underline{76.86}          & +0.89            \\
    BERT-SE$\rm_{\texttt{base}}$ (-w/ LS)                         & \textbf{63.17}                        & \textbf{89.22}                        & 88.83                        & \textbf{80.51}               & \textbf{73.98}          & \textbf{89.29}          & 67.24          & 67.00          & \textbf{\underline{77.41}}          & \textbf{+1.44}            \\
    \hdashline
    BERT-SE$\rm_{\texttt{large}}$ (-w/o LS)                              & \textbf{65.53} & 88.24 & \textbf{89.83} & 83.75 & 79.08 & 87.50 & 67.24 & \textbf{75.00} & \underline{79.52} & +0.40            \\
    BERT-SE$\rm_{\texttt{large}}$ (-w/ LS)        & 64.07 & \textbf{88.48} & 90.12 & \textbf{84.84} & \textbf{79.30} & \textbf{92.86} & \textbf{69.59} & 73.00 & \textbf{\underline{80.28}} & \textbf{+1.16}            \\
    \midrule
    \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{BERT, ``\textbf{random}'' metric}}}  \\

    BERT-SE$\rm_{\texttt{base}}$ (-w/o LS)                            & 63.00 & \textbf{87.50} & 89.07 & \textbf{77.98} & \textbf{74.95} & \textbf{87.50} & \textbf{68.30} & \textbf{62.00} & \textbf{\underline{76.29}} & \textbf{+0.32} \\    
    BERT-SE$\rm_{\texttt{base}}$ (-w/ LS)            &\textbf{63.23} & 87.01 & \textbf{89.12} & 76.17 & 74.83 & 85.70 & 68.00 & \textbf{62.00} & \underline{75.76} & -0.21    \\
    \hdashline
    BERT-SE$\rm_{\texttt{large}}$ (-w/o LS)                              & \textbf{65.28} & 87.74 & 89.68 & 84.12 & 80.1 & 92.9 & 68.8 & 69.00 & \underline{79.70} & +0.58  \\
    BERT-SE$\rm_{\texttt{large}}$ (-w/ LS)                           & 64.59 & \textbf{87.99} & \textbf{89.83} & \textbf{84.84} & \textbf{80.2} & \textbf{94.6} & \textbf{70.2} & \textbf{71.00} & \textbf{\underline{80.41}} & \textbf{+1.29}    \\
    \midrule
    \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{RoBERTa, ``\textbf{loss-based}'' metric}}}  \\ 
    RoBERTa-SE$\rm_{\texttt{base}}$ (-w/o LS)                            & \textbf{64.18}               & 88.48                        & \textbf{90.29}               & 83.39                        & 78.89          & 89.29          & \textbf{73.04}          & 73.00         & \underline{80.07}          & +1.63            \\
    RoBERTa-SE$\rm_{\texttt{base}}$ (-w/ LS)                         & 62.11                        & \textbf{89.71}                       & 90.19                        & \textbf{84.12}               & \textbf{79.39}          & \textbf{92.86}          & 71.40          & \textbf{74.00}          & \textbf{\underline{80.47}}          & \textbf{+2.03}            \\
    \hdashline

    RoBERTa-SE$\rm_{\texttt{large}}$ (-w/o LS)                           & 65.34                        & 90.69                        & \textbf{91.41}                        & \textbf{90.25}                        & \textbf{84.56}          & 94.64          & 69.12          & \textbf{82.00}          & \underline{83.50}          & +1.15            \\
    RoBERTa-SE$\rm_{\texttt{large}}$ (-w/ LS)                       & \textbf{67.80}               & \textbf{91.91}               & 91.20                        & \textbf{90.25}                        & \textbf{84.56}          & \textbf{96.40}          & \textbf{70.53}          & 80.00          & \textbf{\underline{84.08}}          & \textbf{+1.73}            \\
    \midrule
    \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{RoBERTa, ``\textbf{entropy-based}'' metric}}}  \\ 
    RoBERTa-SE$\rm_{\texttt{base}}$ (-w/o LS)                            & 61.95 & \textbf{90.44} & 90.09 & \textbf{83.39} & \textbf{78.53} & \textbf{87.50} & 68.34 & \textbf{75.00} & \underline{79.41} & +0.96            \\
    RoBERTa-SE$\rm_{\texttt{base}}$ (-w/ LS)                         & \textbf{64.06} & 89.71 & \textbf{90.35} & 83.03 & 78.10 & 85.71 & \textbf{69.44} & \textbf{75.00} & \textbf{\underline{79.43}} & \textbf{+0.98}            \\
    \hdashline

    RoBERTa-SE$\rm_{\texttt{large}}$ (-w/o LS)                           & 62.55 & \textbf{90.90} & 91.24 & 89.89 & \textbf{84.19} & \textbf{98.21} & \textbf{71.16} & 81.00 & \textbf{\underline{83.64}} & \textbf{+1.29}            \\
    RoBERTa-SE$\rm_{\texttt{large}}$ (-w/ LS)                       & \textbf{64.17} & 89.71 & \textbf{91.66} & \textbf{90.61} & 84.13 & 96.40 & 70.22 & \textbf{82.00} & \underline{83.61} & +1.26            \\
    \midrule
    \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{RoBERTa, ``\textbf{random}'' metric}}}  \\ 
    RoBERTa-SE$\rm_{\texttt{base}}$ (-w/o LS)                            & 63.78 & 88.73 & \textbf{90.30} & 81.59 & 78.83 & \textbf{89.29} & 69.43 & 68.00 & 78.74 & +0.30            \\
    RoBERTa-SE$\rm_{\texttt{base}}$ (-w/ LS)                         & \textbf{65.61} & \textbf{90.44} & 90.24 & \textbf{83.39} & \textbf{79.36} & 87.50 & \textbf{71.1} & \textbf{72.00} & \textbf{\underline{79.96}} & \textbf{+1.52}       \\
    \hdashline
    RoBERTa-SE$\rm_{\texttt{large}}$ (-w/o LS)      & 62.50 & 89.95 & 91.25 & \textbf{89.89} & \textbf{84.53} & \textbf{92.86} & 70.37 & 63.00 & \underline{80.54} & -1.81           \\
    RoBERTa-SE$\rm_{\texttt{large}}$ (-w/ LS)      & \textbf{63.42} & \textbf{90.20} & \textbf{91.31} & \textbf{89.89} & 84.13 & \textbf{92.86} & \textbf{71.00} & \textbf{80.00} & \textbf{\underline{82.85}} & \textbf{+0.50}          \\
    % RoBERTa-large-entropy                        & 63.2                        & 90.9                        & 91.2                        & 89.9                        & 84.2          & \textbf{98.2}          & \textbf{71.2}          & 81.0          & 83.7          & 1.6            \\
    % RoBERTa-large-entropy-sl                     & 64.2                        & 89.7                        & \textbf{91.7}               & \textbf{90.6}               & 84.1          & 96.4          & 70.2          & \textbf{82.0}          & 83.6          & 1.5  \\         
\bottomrule    
\end{tabular}
}
\caption{Full contrastive results between different masking metrics on the combination of GLUE and SuperGLUE benchmarks. ``-w/o LS'' means that the label smoothing strategy is not used. ``$\Delta$'' denotes the improvement of SE methods compared to the baseline PLMs. Average scores on all tasks are \underline{underlined}. The best results are \textbf{bold}.}
\label{tab:all_results}
\end{table*}

==> [ACL23] SE4PLMs-Camera_Ready/tables/dataset.tex <==
\begin{table*}[h]
\centering
\small
\begin{tabular}{llllcccl}
\toprule
\multicolumn{2}{c}{\textbf{Task}}          & \textbf{\#Train} & \textbf{\#Dev}  & \textbf{\#Class} &\textbf{LR} &\textbf{BSZ} &\textbf{Epochs/Steps} \\ \midrule
\multirow{4}{*}{GLUE}       & CoLA      & 8.5K    & 1,042  & 2   &2e-5  &32  &2668 steps  \\
                            & MRPC        & 3.7K    & 409    & 2   &1e-5  &32  &1148 steps    \\
                            % & STS-B     & 5.7K    & 1,501  & -  &2e-5  &32  &1799 steps     \\
                            & RTE       & 2.5K    & 278    & 2   &1e-5 &16  &2036 steps     \\ \midrule
\multirow{4}{*}{SuperGLUE}  & BoolQ     & 9.4K    & 3,270  & 2  &1e-5    &16  &10 epochs \\
                            & CB        & 250     & 57     & 2   &2e-5  &16  &20 epochs  \\
                            & WiC        & 6K      & 638    & 2  &2e-5    &16  &10 epochs \\
                            & COPA        &400     &100    & 2  &2e-5  &16  &10 epochs   \\ \midrule
\multirow{2}{*}{Commonsense QA} & SQuAD2.0       &130K    &11,873 & -  &3e-5 &12 & 2 epochs      \\
                            & SWAG &73K    &20K  & - &5e-5 &16 & 3 epochs    \\ \midrule
LAMA & Google-RE & \multicolumn{2}{c}{60K} & - & \multicolumn{3}{c}{N/A} \\
\bottomrule
\end{tabular}
\caption{Data statistics and fine-tuning hyper-parameters of all used tasks in this paper. ``Class'' refers to the label class, ``LR'' means the learning rate and ``BSA'' denotes the batch size. Note that the LAMA benchmark is wrapped into a cloze test to probe the PLM without fine-tuning.}
\label{appendix_tab_data}
\end{table*}

==> [ACL23] SE4PLMs-Camera_Ready/tables/iterativeSE.tex <==
\begin{table}[]
    \centering
    \small
    % \resizebox{0.75\columnwidth}{!}
    {
    \begin{tabular}{lccc}
    \toprule
    {\bf GLUE}                  & {\bf $N=1$} & {\bf $N=2$} & {\bf $N=3$}\\
    \midrule
    CoLA	&  63.63   &63.59 &63.60 \\
    MRPC	&  89.50   & 88.23 &88.97 \\
    RTE     &  77.98   &79.42 &78.70 \\ \hdashline
\textit{Avg.} ($\Delta \uparrow$) &  \textcolor[RGB]{0,176,80}{+0.97}   &\textcolor[RGB]{0,176,80}{+1.02} &\textcolor[RGB]{0,176,80}{+1.03} \\ 
    \bottomrule
    \end{tabular}}
    \caption{Performance for different iterations $N$ on BERT-SE$_{\texttt{base}}$. ``\textit{Avg.} ($\Delta \uparrow$)'' indicates the relative improvement against the vanilla BERT$_{\texttt{base}}$.}
    \label{tab:iterations}
\end{table}


==> [ACL23] SE4PLMs-Camera_Ready/tables/lama.tex <==
\begin{table}[t]
\centering
\small
\scalebox{0.84}{
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{l}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{Google-RE (LAMA)}}                                                     & \multirow{2}{*}{\textbf{\underline{Avg.}}} \\ \cmidrule(lr){2-4}
\multicolumn{1}{c}{}                        & date-birth      & place-birth     & place-death     &                       \\ \midrule
% \multicolumn{5}{l}{\textit{Performance in terms of Mean Reciprocal Rank (MRR)}} \\ \midrule
RoBERTa$\rm_{\texttt{base}}$                               & 5.51                 & 11.52                & 2.68                 & \underline{6.57}                \\
% \brobertacont                           & 5.85                 & 12.37                & 3.80                  & 23.20                 & \textbf{25.12}       & \textbf{20.53}       & \underline{15.15}                 \\ \hdashline
% \brobertasse                            & 6.00                 & 13.03                & 9.26                 & 22.34                & 23.20                & 17.39                & \underline{15.20}                 \\
\bf RoBERTa-SE$\rm_{\texttt{base}}$                           & \textbf{6.35}        & \textbf{15.16}       & \textbf{9.61}                       & \textbf{\underline{10.37}}        \\ 
% \midrule
% \multicolumn{5}{l}{\textit{Performance in terms of Mean precision at one (P@1)}} \\ \midrule
% % \broberta                               & 0.96                 & 7.09                 & 1.40                 & 14.16                & 16.85                & \textbf{10.75}       & \underline{8.54}                  \\
% RoBERTa$\rm_{\texttt{base}}$                           & \textbf{1.47}        & 6.30                 & 1.71                                & -                  \\ 
% % \hdashline
% % \brobertasse                            & 1.22                 & 6.05                 & 5.27                 & 13.77                & 15.60                & 9.32                 & \underline{8.54}                  \\
% RoBERTa-SE$\rm_{\texttt{base}}$                           & 1.41                 & \textbf{8.80}        & \textbf{6.51}                        & \textbf{+2.41}    \\
\bottomrule
\end{tabular}
}
\caption{Performance of our $\mathbb{SE}$ on LAMA~\cite{petroni2019language} to probe the factual knowledge.
% The best results are \textbf{bold}. 
% It shows that SE helps the PLMs on the learning of knowledge.
}
\label{tab_lama}
\end{table}

==> [ACL23] SE4PLMs-Camera_Ready/tables/main_results.tex <==
% Please add the following required packages to your document preamble:
\begin{table*}[]
\centering
\scalebox{0.91}{
    \begin{tabular}{lccccccccc}
    \toprule
    \multicolumn{1}{c}{}                         &\bf CoLA                        &\bf MRPC                                              &\bf RTE                         &\bf BoolQ         &\bf CB            &\bf WiC           &\bf COPA          & \multicolumn{2}{c}{\bf Score}      \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-8} \cmidrule(lr){9-10} 
    \multicolumn{1}{l}{\multirow{-2}{*}{\bf Method}} & \textit{Mcc.}               & \textit{Acc.}                             & \textit{Acc.}               & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \textit{\underline{Avg.}} & \textit{$\Delta$ ($\uparrow$)} \\
    \midrule
    \multicolumn{10}{l}{\textit{Performance of Different Masking Strategies}}  \\ \midrule
    BERT$\rm_{\texttt{base}}$                               & 62.33                        & 88.97                                                & 76.89                        & \textbf{75.05}          & 85.71          & 66.77          & 63.00          & \underline{74.10}          & --              \\
    \hdashline
    \quad -w/ Entity-level masking & 60.06 & 88.73 & 76.53 & 74.77 & 87.50 & 66.61 & 65.00 & 74.17          & \textcolor[RGB]{0,176,80}{+0.07}             \\
    \quad -w/ Span-level masking & 61.41 & 88.48 & \textbf{78.34} & 74.28 & 87.50 & 67.40 & 65.00 & 74.63         & \textcolor[RGB]{0,176,80}{+0.53}             \\
    \quad -w/ PMI-based masking & 61.09 & 88.24 & 76.90 & 74.25 & 87.50 & 66.61 & 65.00 & 74.23           & \textcolor[RGB]{0,176,80}{+0.13}             \\
    \quad -w/ Self-questioning & \textbf{63.78} & 87.99 & \textbf{78.34} & 74.13 & 85.71 & \textbf{67.87} & \textbf{66.00} & 74.83         & \textcolor[RGB]{0,176,80}{+0.73}             \\
    \textbf{BERT-SE}$\rm_{\texttt{base}}$                         & 63.63 & \textbf{89.50} & 77.98 & 74.37 & \textbf{89.29} & 67.40 & \textbf{66.00} & \textbf{\underline{75.45}} & \textcolor[RGB]{0,176,80}{\textbf{+1.35}}            \\
    \midrule
    \multicolumn{10}{l}{\textit{Performance upon More Discriminative PLMs}}  \\ \midrule
    BERT$\rm_{\texttt{large}}$                               & 63.00                        & 87.25                                              & 83.80                        & 78.40          & 91.07         & 67.24          & 72.00          & \underline{77.54}          & --              \\
    \textbf{BERT-SE}$\rm_{\texttt{large}}$                           & \textbf{65.66}               & \textbf{88.23}                                              & \textbf{85.20}               & \textbf{80.18}          & \textbf{92.86}          & \textbf{68.34}          & \textbf{78.00}          & \textbf{\underline{79.78}}          & \textcolor[RGB]{0,176,80}{\textbf{+2.24}}            \\
    \hdashline
    RoBERTa$\rm_{\texttt{base}}$                            & 62.00                        & \textbf{90.20}                                                & 83.12                        & 78.72          & 83.93          & 69.12          & 70.00          & \underline{76.72}          & --              \\
    \textbf{RoBERTa-SE}$\rm_{\texttt{base}}$                         & \textbf{62.11}                        & 89.71                                               & \textbf{84.12}               & \textbf{79.39}          & \textbf{92.86}          & \textbf{71.40}          & \textbf{74.00}          & \textbf{\underline{79.08}}          & \textcolor[RGB]{0,176,80}{\textbf{+2.36}}            \\
    \hdashline
    RoBERTa$\rm_{\texttt{large}}$                            & 64.73                        & 90.69                                               & 88.44                        & 84.37          & 91.07          & 69.90          & 78.00          & \underline{81.03}          & --              \\
    \textbf{RoBERTa-SE}$\rm_{\texttt{large}}$                       & \textbf{67.80}               & \textbf{91.91}                                    & \textbf{90.25}                        & \textbf{84.56}          & \textbf{96.40}          & \textbf{70.53}          & \textbf{80.00}          & \textbf{\underline{83.06}}          & \textcolor[RGB]{0,176,80}{\textbf{+2.03}}            \\       
\bottomrule    
\end{tabular}
}
\caption{Comparison between our $\mathbb{SE}$ and the vanilla method applied to all PLMs on the combination of GLUE and SuperGLUE benchmarks. Average scores on all tasks are \underline{underlined}. The best results are given in \textbf{bold}. ``$\Delta$'' denotes the improvement of $\mathbb{SE}$ methods compared to the baseline PLMs. 
% It shows that SE method yields consistent improvements among all PLMs, indicating the effectiveness and universality of SE method.
}
\label{tab:main1}
\end{table*}

==> [ACL23] SE4PLMs-Camera_Ready/tables/main_results2.tex <==

\begin{table}[t]
\scalebox{0.87}{
    \begin{tabular}{lcccc}
\toprule
    \multicolumn{1}{l}{\multirow{2}{*}{\bf Method}} & \multicolumn{2}{c}{\bf SQuAD2.0}    &\bf  SWAG           &\bf \multirow{2}{*}{\underline{Avg.}} \\
    \cmidrule(){2-4}
    \multicolumn{1}{c}{}                        & \textit{EM}             & \textit{F1}             & \textit{Acc.}           &                       \\
    \midrule
    BERT$\rm_{\texttt{base}}$                              & 72.18          & 75.07          & 77.53          & \underline{74.93}                 \\
    \textbf{BERT-SE}$\rm_{\texttt{base}}$                           & \textbf{72.89}          & \textbf{75.64} & \textbf{77.91}          & \textbf{\underline{75.48}}        \\
    \hdashline
    BERT$\rm_{\texttt{large}}$                            & 81.35          & 84.38          & 83.40          & \underline{83.04}                 \\
    \textbf{BERT-SE}$\rm_{\texttt{large}}$                       & \textbf{81.94} & \textbf{85.00} & \textbf{83.61}          & \textbf{\underline{83.52}}       
\\ \midrule
    RoBERTa$\rm_{\texttt{base}}$                              & 78.79          & 81.92          & 79.69          & \underline{80.13}                 \\
    \textbf{RoBERTa-SE}$\rm_{\texttt{base}}$                           & \textbf{79.41}          & \textbf{82.55} & \textbf{79.88}          & \textbf{\underline{80.61}}        \\
    \hdashline
    RoBERTa$\rm_{\texttt{large}}$                            & 84.70          & 87.65          & 84.34          & \underline{85.56}                 \\
    \textbf{RoBERTa-SE}$\rm_{\texttt{large}}$                       & \textbf{85.03} & \textbf{87.93} & \textbf{84.54}          & \textbf{\underline{85.83}} 
    \\

\bottomrule    
\end{tabular}
}
\caption{Performance on SQuAD2.0~\cite{rajpurkar2018know} and SWAG~\cite{zellers-etal-2018-swag} dev sets. 
% We observe that, with the help of the SE mechanism, PLMs perform better on knowledge-intense tasks.
}
\label{tab:main2}
\end{table}

==> [ACL23] SE4PLMs-Camera_Ready/tables/metric_ablation.tex <==
\begin{table*}[]
\centering
\scalebox{0.745}{
\begin{tabular}{ccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{BERT}$\rm_{\texttt{base}}$}             & \multicolumn{2}{c}{\textbf{BERT}$\rm_{\texttt{large}}$}               & \multicolumn{2}{c}{\textbf{\textsc{RoBERTa}}$\rm_{\texttt{base}}$}            & \multicolumn{2}{c}{\textbf{\textsc{RoBERTa}}$\rm_{\texttt{large}}$}   & \multicolumn{2}{c}{\textbf{Avg.}}     \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} 
  & -w/o TLS                  & -w/ TLS                  & -w/o TLS                  & -w/ TLS                  & -w/o TLS                  & -w/ TLS                  & -w/o TLS                  & -w/ TLS    
  & -w/o TLS                  & -w/ TLS \\
\midrule
Baseline                    & \multicolumn{2}{c}{75.97}                    & \multicolumn{2}{c}{79.12}                    & \multicolumn{2}{c}{78.44}                    & \multicolumn{2}{c}{82.35}     & \multicolumn{2}{c}{\underline{78.97}}                 \\ 
% Cont                    & \multicolumn{2}{c}{+0.62}                    & \multicolumn{2}{c}{+0.44}                    & \multicolumn{2}{c}{+0.27}                    & \multicolumn{2}{c}{+0.23}     & \multicolumn{2}{c}{\underline{+0.39}}                 \\ 
\hdashline
\multicolumn{11}{l}{masking metric in SE}  \\
\multicolumn{1}{l}{\quad -- random}  &+0.32  &-0.21  &+0.58  &+1.29  &+0.30  &+1.52  &-1.81  &+0.50   &\underline{-0.15}  &\underline{+0.78}  \\	
\multicolumn{1}{l}{\quad -- loss-based}                 & +1.02                 & +1.18              & +0.83                 & \textbf{+1.92}                         & +1.63                  & \textbf{+2.03}                  & +1.15                 & \textbf{+1.73}   & \underline{+1.16}                 & \underline{\textbf{+1.72}}                \\
\multicolumn{1}{l}{\quad -- entropy-based}        & +0.89                 & \textbf{+1.44}                & +0.40     & +1.16                 & 0.96                   & +0.98                  & +1.29                 & +1.26        & \underline{+0.89}                & \underline{+1.21}    \\
\bottomrule
\end{tabular}
}
\caption{Ablation study of the masking metric used in our SE methods on the combination of GLUE and SuperGLUE benchmarks. For simplicity, we show the overall score and relative gains in this table. The full results can be found in Appendix~\ref{appendix_full} (Table~\ref{tab:all_results}).}
\label{tab:ablation1}
\end{table*}

==> [ACL23] SE4PLMs-Camera_Ready/tables/statistic_analysis.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{ccc}
    \toprule
    \textbf{JS($P_1||P_2$}) & \textbf{KL($P_2||P_1$)} & \textbf{KL($P_1||P_2$)} \\
    \midrule
    0.1681   &0.3875 &0.7506 \\ 
    \bottomrule
    \end{tabular}
    \caption{Distribution difference between vocabulary distributions selected by Correctness-based ``$P_1$'' and Confidence-based ``$P_2$'' metrics. BERT-SE$\rm_{\texttt{large}}$ is used.}
    \label{tab:statistic}
\end{table}


==> tables/all_results2.tex <==
% Please add the following required packages to your document preamble:
\begin{table*}[]
\centering
\scalebox{0.85}{
    \begin{tabular}{lcccccccccc}
    \toprule
    \multicolumn{1}{c}{}                         & CoLA                        & MRPC                        & STS-B                       & RTE                         & BoolQ         & CB            & WiC           & COPA          & \multicolumn{2}{c}{Score}      \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-11} 
    \multicolumn{1}{l}{\multirow{-2}{*}{Method}} & \textit{Mcc.}               & \textit{Acc.}               & \textit{Pear.}              & \textit{Acc.}               & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \textit{Acc.} & \textit{\underline{Avg.}} & \textit{$\Delta$} \\
    \midrule \midrule
    \multicolumn{11}{l}{{\textbf{\textit{Baseline PLMs}}}}  \\
    \quad BERT$\rm_{\texttt{base}}$                                & 62.33                        & 88.97                        & 89.04                       & 76.89                        & 75.05          & 85.71          & 66.77          & 63.00          & \underline{75.97}          & -- \\
    \quad BERT$\rm_{\texttt{large}}$                               & 63.00                        & 87.25                        & 90.20                        & 83.80                        & 78.40          & 91.07         & 67.24          & 72.00          & \underline{79.12}          & --              \\
    \quad RoBERTa$\rm_{\texttt{base}}$                            & 62.00                        & 90.20                        & 90.45                        & 83.12                        & 78.72          & 83.93          & 69.12          & 70.00          & \underline{78.44}          & --              \\
    \quad RoBERTa$\rm_{\texttt{large}}$                            & 64.73                        & 90.69                        & 91.62                        & 88.44                        & 84.37          & 91.07          & 69.90          & 78.00          & \underline{82.35}          & --              \\ \midrule
    \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{BERT, ``\textbf{loss-based}'' metric}}}  \\
    BERT-SE$\rm_{\texttt{base}}$ (-w/o LS)                            & \textbf{64.78} & 87.99 & \textbf{89.08} & \textbf{78.34} & 74.13 & 85.71 & \textbf{67.87} & \textbf{68.00} & \underline{76.99} & +1.02            \\
    BERT-SE$\rm_{\texttt{base}}$ (-w/ LS)                         & 63.63 & \textbf{89.50} & 89.03 & 77.98 & \textbf{74.37} & \textbf{89.29} & 67.40 & 66.00 & \textbf{\underline{77.15}} & \textbf{+1.18}            \\
    \hdashline
    BERT-SE$\rm_{\texttt{large}}$ (-w/o LS)                              & 64.14                        & \textbf{88.73}               & \textbf{89.95}               & 84.83                        & 79.93          & \textbf{92.86}          & 68.18          & 71.00          & \underline{79.95}          & +0.83            \\
    BERT-SE$\rm_{\texttt{large}}$ (-w/ LS)                           & \textbf{65.66}               & 88.23                        & 89.84                        & \textbf{85.20}               & \textbf{80.18}          & \textbf{92.86}          & \textbf{68.34}          & \textbf{78.00}          & \textbf{\underline{81.04}}          & \textbf{+1.92}            \\
    \midrule
    \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{BERT, ``\textbf{entropy-based}'' metric}}}  \\ 

    BERT-SE$\rm_{\texttt{base}}$ (-w/o LS)                            & 62.82                        & 88.24                        & \textbf{88.86}                        & 77.98                        & 73.43          & 87.50          & \textbf{68.03}          & \textbf{68.00}          & \underline{76.86}          & +0.89            \\
    BERT-SE$\rm_{\texttt{base}}$ (-w/ LS)                         & \textbf{63.17}                        & \textbf{89.22}                        & 88.83                        & \textbf{80.51}               & \textbf{73.98}          & \textbf{89.29}          & 67.24          & 67.00          & \textbf{\underline{77.41}}          & \textbf{+1.44}            \\
    \hdashline
    BERT-SE$\rm_{\texttt{large}}$ (-w/o LS)                              & \textbf{65.53} & 88.24 & \textbf{89.83} & 83.75 & 79.08 & 87.50 & 67.24 & \textbf{75.00} & \underline{79.52} & +0.40            \\
    BERT-SE$\rm_{\texttt{large}}$ (-w/ LS)        & 64.07 & \textbf{88.48} & 90.12 & \textbf{84.84} & \textbf{79.30} & \textbf{92.86} & \textbf{69.59} & 73.00 & \textbf{\underline{80.28}} & \textbf{+1.16}            \\
    \midrule
    \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{BERT, ``\textbf{random}'' metric}}}  \\

    BERT-SE$\rm_{\texttt{base}}$ (-w/o LS)                            & 63.00 & \textbf{87.50} & 89.07 & \textbf{77.98} & \textbf{74.95} & \textbf{87.50} & \textbf{68.30} & \textbf{62.00} & \textbf{\underline{76.29}} & \textbf{+0.32} \\    
    BERT-SE$\rm_{\texttt{base}}$ (-w/ LS)            &\textbf{63.23} & 87.01 & \textbf{89.12} & 76.17 & 74.83 & 85.70 & 68.00 & \textbf{62.00} & \underline{75.76} & -0.21    \\
    \hdashline
    BERT-SE$\rm_{\texttt{large}}$ (-w/o LS)                              & \textbf{65.28} & 87.74 & 89.68 & 84.12 & 80.1 & 92.9 & 68.8 & 69.00 & \underline{79.70} & +0.58  \\
    BERT-SE$\rm_{\texttt{large}}$ (-w/ LS)                           & 64.59 & \textbf{87.99} & \textbf{89.83} & \textbf{84.84} & \textbf{80.2} & \textbf{94.6} & \textbf{70.2} & \textbf{71.00} & \textbf{\underline{80.41}} & \textbf{+1.29}    \\
    \midrule
    \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{RoBERTa, ``\textbf{loss-based}'' metric}}}  \\ 
    RoBERTa-SE$\rm_{\texttt{base}}$ (-w/o LS)                            & \textbf{64.18}               & 88.48                        & \textbf{90.29}               & 83.39                        & 78.89          & 89.29          & \textbf{73.04}          & 73.00         & \underline{80.07}          & +1.63            \\
    RoBERTa-SE$\rm_{\texttt{base}}$ (-w/ LS)                         & 62.11                        & \textbf{89.71}                       & 90.19                        & \textbf{84.12}               & \textbf{79.39}          & \textbf{92.86}          & 71.40          & \textbf{74.00}          & \textbf{\underline{80.47}}          & \textbf{+2.03}            \\
    \hdashline

    RoBERTa-SE$\rm_{\texttt{large}}$ (-w/o LS)                           & 65.34                        & 90.69                        & \textbf{91.41}                        & \textbf{90.25}                        & \textbf{84.56}          & 94.64          & 69.12          & \textbf{82.00}          & \underline{83.50}          & +1.15            \\
    RoBERTa-SE$\rm_{\texttt{large}}$ (-w/ LS)                       & \textbf{67.80}               & \textbf{91.91}               & 91.20                        & \textbf{90.25}                        & \textbf{84.56}          & \textbf{96.40}          & \textbf{70.53}          & 80.00          & \textbf{\underline{84.08}}          & \textbf{+1.73}            \\
    \midrule
    \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{RoBERTa, ``\textbf{entropy-based}'' metric}}}  \\ 
    RoBERTa-SE$\rm_{\texttt{base}}$ (-w/o LS)                            & 61.95 & \textbf{90.44} & 90.09 & \textbf{83.39} & \textbf{78.53} & \textbf{87.50} & 68.34 & \textbf{75.00} & \underline{79.41} & +0.96            \\
    RoBERTa-SE$\rm_{\texttt{base}}$ (-w/ LS)                         & \textbf{64.06} & 89.71 & \textbf{90.35} & 83.03 & 78.10 & 85.71 & \textbf{69.44} & \textbf{75.00} & \textbf{\underline{79.43}} & \textbf{+0.98}            \\
    \hdashline

    RoBERTa-SE$\rm_{\texttt{large}}$ (-w/o LS)                           & 62.55 & \textbf{90.90} & 91.24 & 89.89 & \textbf{84.19} & \textbf{98.21} & \textbf{71.16} & 81.00 & \textbf{\underline{83.64}} & \textbf{+1.29}            \\
    RoBERTa-SE$\rm_{\texttt{large}}$ (-w/ LS)                       & \textbf{64.17} & 89.71 & \textbf{91.66} & \textbf{90.61} & 84.13 & 96.40 & 70.22 & \textbf{82.00} & \underline{83.61} & +1.26            \\
    \midrule
    \multicolumn{11}{c}{\cellcolor{lightgray}{\textit{RoBERTa, ``\textbf{random}'' metric}}}  \\ 
    RoBERTa-SE$\rm_{\texttt{base}}$ (-w/o LS)                            & 63.78 & 88.73 & \textbf{90.30} & 81.59 & 78.83 & \textbf{89.29} & 69.43 & 68.00 & 78.74 & +0.30            \\
    RoBERTa-SE$\rm_{\texttt{base}}$ (-w/ LS)                         & \textbf{65.61} & \textbf{90.44} & 90.24 & \textbf{83.39} & \textbf{79.36} & 87.50 & \textbf{71.1} & \textbf{72.00} & \textbf{\underline{79.96}} & \textbf{+1.52}       \\
    \hdashline
    RoBERTa-SE$\rm_{\texttt{large}}$ (-w/o LS)      & 62.50 & 89.95 & 91.25 & \textbf{89.89} & \textbf{84.53} & \textbf{92.86} & 70.37 & 63.00 & \underline{80.54} & -1.81           \\
    RoBERTa-SE$\rm_{\texttt{large}}$ (-w/ LS)      & \textbf{63.42} & \textbf{90.20} & \textbf{91.31} & \textbf{89.89} & 84.13 & \textbf{92.86} & \textbf{71.00} & \textbf{80.00} & \textbf{\underline{82.85}} & \textbf{+0.50}          \\
    % RoBERTa-large-entropy                        & 63.2                        & 90.9                        & 91.2                        & 89.9                        & 84.2          & \textbf{98.2}          & \textbf{71.2}          & 81.0          & 83.7          & 1.6            \\
    % RoBERTa-large-entropy-sl                     & 64.2                        & 89.7                        & \textbf{91.7}               & \textbf{90.6}               & 84.1          & 96.4          & 70.2          & \textbf{82.0}          & 83.6          & 1.5  \\         
\bottomrule    
\end{tabular}
}
\caption{Full contrastive results between different masking metrics on the combination of GLUE and SuperGLUE benchmarks. ``-w/o LS'' means that the label smoothing strategy is not used. ``$\Delta$'' denotes the improvement of SE methods compared to the baseline PLMs. Average scores on all tasks are \underline{underlined}. The best results are \textbf{bold}.}
\label{tab:all_results}
\end{table*}

==> tables/metric_ablation.tex <==
\begin{table*}[]
\centering
\scalebox{0.745}{
\begin{tabular}{ccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{BERT}$\rm_{\texttt{base}}$}             & \multicolumn{2}{c}{\textbf{BERT}$\rm_{\texttt{large}}$}               & \multicolumn{2}{c}{\textbf{\textsc{RoBERTa}}$\rm_{\texttt{base}}$}            & \multicolumn{2}{c}{\textbf{\textsc{RoBERTa}}$\rm_{\texttt{large}}$}   & \multicolumn{2}{c}{\textbf{Avg.}}     \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} 
  & -w/o TLS                  & -w/ TLS                  & -w/o TLS                  & -w/ TLS                  & -w/o TLS                  & -w/ TLS                  & -w/o TLS                  & -w/ TLS    
  & -w/o TLS                  & -w/ TLS \\
\midrule
Baseline                    & \multicolumn{2}{c}{75.97}                    & \multicolumn{2}{c}{79.12}                    & \multicolumn{2}{c}{78.44}                    & \multicolumn{2}{c}{82.35}     & \multicolumn{2}{c}{\underline{78.97}}                 \\ 
% Cont                    & \multicolumn{2}{c}{+0.62}                    & \multicolumn{2}{c}{+0.44}                    & \multicolumn{2}{c}{+0.27}                    & \multicolumn{2}{c}{+0.23}     & \multicolumn{2}{c}{\underline{+0.39}}                 \\ 
\hdashline
\multicolumn{11}{l}{masking metric in SE}  \\
\multicolumn{1}{l}{\quad -- random}  &+0.32  &-0.21  &+0.58  &+1.29  &+0.30  &+1.52  &-1.81  &+0.50   &\underline{-0.15}  &\underline{+0.78}  \\	
\multicolumn{1}{l}{\quad -- loss-based}                 & +1.02                 & +1.18              & +0.83                 & \textbf{+1.92}                         & +1.63                  & \textbf{+2.03}                  & +1.15                 & \textbf{+1.73}   & \underline{+1.16}                 & \underline{\textbf{+1.72}}                \\
\multicolumn{1}{l}{\quad -- entropy-based}        & +0.89                 & \textbf{+1.44}                & +0.40     & +1.16                 & 0.96                   & +0.98                  & +1.29                 & +1.26        & \underline{+0.89}                & \underline{+1.21}    \\
\bottomrule
\end{tabular}
}
\caption{Ablation study of the masking metric used in our SE methods on the combination of GLUE and SuperGLUE benchmarks. For simplicity, we show the overall score and relative gains in this table. The full results can be found in Appendix~\ref{appendix_full} (Table~\ref{tab:all_results}).}
\label{tab:ablation1}
\end{table*}
